Generalization Ability of Wide Neural Networks on $\mathbb{R}$

We perform a study on the generalization ability of the wide two-layer ReLU neural network on $\mathbb{R}$. We first establish some spectral properties of the neural tangent kernel (NTK): $a)$ $K_{d}$, the NTK defined on $\mathbb{R}^{d}$, is positive definite; $b)$ $\lambda_{i}(K_{1})$, the $i$-th largest eigenvalue of $K_{1}$, is proportional to $i^{-2}$. We then show that: $i)$ when the width $m\rightarrow\infty$, the neural network kernel (NNK) uniformly converges to the NTK; $ii)$ the minimax rate of regression over the RKHS associated to $K_{1}$ is $n^{-2/3}$; $iii)$ if one adopts the early stopping strategy in training a wide neural network, the resulting neural network achieves the minimax rate; $iv)$ if one trains the neural network till it overfits the data, the resulting neural network can not generalize well. Finally, we provide an explanation to reconcile our theory and the widely observed ``benign overfitting phenomenon''.

==> ES.tex <==
%Add a paragraph for cohesion
We have shown in Theorem \ref{thm:bad_gen} that, when the equally-distanced data is fitted, the lazy trained 1-hidden neural network can be approximated by linear interpolation. Thus, a lazy trained overfitted neural network can not generalize well. That means the training process should be stopped before the network overfits the data. 


\subsection{Wide neural networks are minimax optimal with early stopping}

% Raskutti et al. \cite{raskutti2014early}  
Lin et al. \cite{lin2020optimal} have considered the regression problem (Equation \eqref{equation:true_model}). They investigated the generalization ability of the solution obtained by gradient descent method with $0\in \mathcal{H}_{\Phi}$ as the initialization point(function), and showed that a properly chosen early stopping strategy leads to a minimax optimal solution if we know the decay rate of eigenvalues of the kernel. %Add more words

\begin{theorem}\label{thm:K_decay_rate} 
    Let $\{\lambda_{j}, j=0, 1,2,\cdots\}$ be the eigenvalues associated to the NTK $K$ on $[0,1]$. Then we have 
    \begin{equation}
        \frac{1}{2\pi^3} \frac{1}{j^{2}}\leq \lambda_j \leq \frac{14}{\pi^3} \frac{1}{j^{2}}, j=1,2,...
    \end{equation}
\end{theorem}
%Add remark how to prove 
\begin{remark}
The kernel $K$ can be reformulated as the sum of two kernels. One is the main kernel, offering the main properties of NTK. And the proof of Theorem \ref{thm:K_decay_rate} is based on the bounds of the eigenvalues associated to the main kernel. Theorem \ref{thm:K_decay_rate} clearly shows the upper and lower bounds of the eigenvalues and indicates the size of the RKHS of NTK.  
\end{remark}

Proposition \ref{prop:early:stopping} is a direct consequence from \cite{lin2020optimal} by applying Theorem \ref{thm:K_decay_rate}.
  
%It may need more efforts to establish them and will be one of our main focus in future work.

%It is proved in \cite{hu2021regularization} that $\lambda_{i}\asymp i^{-d/(d-1)}$ when the NTK is defined on the sphere $\mathbb{S}^{d-1}$. 

%then it's natural to assume the following
%    for all RKHS restricted to uniform distribution on the sphere, spherical harmonic functions are common basis. The inclusion relations of RKHS only depend on the eigenvalue decay. Faster the decay, larger the RKHS because functions in it are smoother. \cite{lukic2001stochastic} show the necessary and sufficient conditions for draws from a Gaussian process with kernel $\Sigma$ lie in the RKHS of kernel $K$ with probability one are the inclusion operator is Hilbert-Schmidt. We will keep work on proving this assumption in future work. 


% \begin{lemma}[Infinite width linearized neural networks using early stopping are minimax optimal]\label{inf-lin-opt}
%     \[
%         \mathbb{E}\lVert f_{\mathsf{lin},t_{\star}}^{m=\infty,\mathbf{z}}-f_{\star}\rVert_{L^2(\mu)}^2=\mathcal{O}(n^{-2/3})
%     \]
% \end{lemma}


\begin{proposition}[Optimality of early stopping]\label{prop:early:stopping} 
For the NTK regression, if we stop the training process at $t_{\star}=c n^{2/3}$, the resulting (neural network) $f_{t_{\star}}^{\NTK}$ satisfies that
\begin{equation}
     \lVert f_{t_{\star}}^{\NTK}-f_{\star}\rVert^{2} \leq cn^{-2/3},
\end{equation}
with high probability,
which matches the minimax lower bounds, since we have
\begin{equation}
    \inf_{\hat{f}}\sup_{f_{\star}\in\mathcal{H}_{K},\lVert f_{\star}\rVert\leq R}\Expc\lVert \hat{f}-f_{\star}\rVert^{2} \geq cn^{-2/3}.
\end{equation}
\end{proposition}

Combining Proposition \ref{prop:early:stopping} and Proposition \ref{prop: generalization closeness}, Corollary \ref{cor: nn early stopping} follows, indicating the overparameterized two-layer neural network with early stopping is minimax rate optimal.
%\begin{corollary}\label{cor: nn early stopping}
%    If $m$ is sufficiently large, then
%    \begin{equation}
%    \lVert f_{\bm{\theta}(t_{\star})}(x)-f_{\star}\rVert^{2} \leq Cn^{-2/3},
%    \end{equation}
%    i.e., the fact that neural network using early stopping is minimax optimal holds with probability at least $1-P(m)$ over random initialization and with high probability over the training data.
%\end{corollary}

\begin{corollary}\label{cor: nn early stopping}
    If $m$ is sufficiently large, then
    \begin{equation}
    \lVert f_{\bm{\theta}(t_{\star})}-f_{\star}\rVert^{2} \leq cn^{-2/3},
    \end{equation}
    with probability at least $1-P(m)$ over random initialization and with high probability over the training data.
\end{corollary}

% $\{\lambda_{i}\geq Ci^{-2}, i=1,2,\cdots\}$ implies that there is a minimax lower bound on the risk  . i.e., For any estimate $\widehat{f}$ of $f_{\star}$ based of the $n$ i.i.d. samples $\{(x_{i},y_{i})\}_{i=1,\cdots,n}$, one has
% \begin{align}
%     \sup_{f_{\star} \in \mathcal{H}_{K}}
%               \int_{0}^{1} ( \widehat{f}-f_{\star})^2 dx \leq C\sigma^{2}n^{-2/3}.
% \end{align}
% In other words, the early stopped $f^{NTK}_{t_{\star}}$ achieves the minimax rate.

The statement in Section \ref{sec:main_result} that neural network that overfitted neural network cannot generalize well seems to contradict the observation (S). However, we realize that it might be caused by the subtle difference between zero training label error and zero training loss. In other words, the training till zero training label error is actually stopped earlier than the time till interpolating the data. We present this subtle difference through the following illustrative example.

\begin{figure}[h]
\centering
\includegraphics[scale=0.4]{100accuracy_vs_interpolation}
\caption{Overfitting vs. 100 \% label accuracy: 4 training data points $\{(0,0),(\frac{1}{3},1),(\frac{2}{3},0), (1,1) \}$. We use gradient descent to train a one-hidden-layer neural network with large width $m=1000$. Compared with the interpolation regime, the loss in the epoch with 100 \% label accuracy is still large. The function in the epoch with 100 \% label accuracy is also far different from the function in the interpolation regime.}
\label{fig: interpolation vs acc}
\end{figure}

Although we realize the stopping time with zero training label error can be an implicit early stopping, we find that the occurrence of this implicit early stopping depends on the scale of the noise(the fraction of label corruption). In other words, the signal strength of data plays a significant role in this case.

\subsection{On the role of signal strength}

Proposition \ref{prop:early:stopping} shows that a carefully chosen early stopping time will produce a neural network  achieving the minimax rate. 
Zhang et al. \cite{zhang2016understanding} observed the implicit early stopping strategy, stopping the training process when the 100\% label accuracy is reached, can generalize well. One may speculate that the implicit early stopping time is the optimal stopping time that appeared in Proposition \ref{prop:early:stopping}. However, this sounds too good to be true. In fact, Zhang et al. \cite{zhang2016understanding} have discussed the role of some explicit early stopping strategies in training neural networks. They observed that: 1. early stopping indeed makes generalization better on ImageNet and 2. early stopping does not help much on CIFAR10. These observations made the effects of the implicit early stopping elusive. We can not simply claim that an implicit early-stopping strategy would produce a rate-optimal neural network.

We hypothesized that signal strength plays an indispensable role in the success of implicit early-stopping strategies. More precisely, when the signal strength is strong enough, the implicit early stopping strategy will produce a stopping time near the optimal stopping time $t_{\star}$; and when the signal strength is deteriorated (e.g., after performing label corruption procedure), the implicit early stopping strategy will produce a stopping time far from the optimal stopping time $t_{\star}$. 

%Talk about what is the signal strength: Smoothness and the scale of noise
%We will talk about the two reasons why the overfitted neural network can still generalize:

\subsection{Noise of data}

%Define the scale of noise
In Section \ref{intro}, we assume the noise $\epsilon\sim N(0,\sigma)$, which iss too good to be true in real cases. Nevertheless, we can still believe there is a ground true function $f^*(x)$ behind the data. Thus, we can define the gap between the label and the ground true function as noise, i.e.,
\begin{equation}
    \epsilon = y - f_{\star}(x).
\end{equation}
In binary classification problems, the true label can be defined as
\begin{equation}
    y_{\text{true}}=\bm{1}_{f_{\star}(x)>0.5}.
\end{equation}
The labels of data $y$ are possibly different from the true labels $y_{true}$.  If the noise does not affect the true label, i.e., $y=y_{\text{true}}$, then the noise is considered as a small noise. For example, $f_{\star}(x_1)=0.1$ and the label $y_1=0$ and $f^*(x_2)=0.9$ and the label $y_1=1$. These two data points has small noise since the gap does not affect the true labels of $f_{\star}(x_1)$ and $f_{\star}(x_2)$. However, if the noise affects the true label, that means the label corruption happens. For example, if $f_{\star}(x_3)=0.1$ but the label $y_3=1$, that means the noise affects the true label of $f_{\star}(x_3)$.

In general, the epoch with the maximum accuracy on validation set or the long-time unchanged training loss is commonly chosen as the stopping time. In this case, early stopping is potentially used. If the neural network is trained until it reach 100\% training accuracy, we tend to believe the network violates the conditions of early stopping and can not have good performance on testing set. However, if the noise is small, 100\% training accuracy does not mean the sufficient small loss(Figure \ref{fig: interpolation vs acc}). The neural network may have large training loss even if it reaches 100\% training accuracy, which means the training process is early stopped before the interpolation regime.

If the noise is large, the 100\%-training-accuracy neural network can not have good generalization. From Figure \ref{fig: MLP_diff_noise_mse} and \ref{fig: Alexnet_cifar10_diff_noise_ce}, we can find that as the percentage of label corruption is increasing, the training time to 100\% training accuracy is increasing. Moreover, the generalization gap between `100\% training accuracy' and `best generalization' becomes larger. In these cases, explicit early stopping(e.g. cross validation) is still significant to the generalization of the model.

In summary, we finally filled the last piece of jigsaw in reconciling the controversial observation (S) and the bias-variance trade-off doctrine in classical statistical learning theory.

==> LI.tex <==
In Section \ref{ntk:recollect}, we have mentioned $f_{t}^{m}$ can be effectively approximated by $f_{t}^{NTK}$. So we will focus on the asymptotic behaviour of $f_{t}^{NTK}(x)$ from now on. We will give an example over one dimensional data showing that $f_{t}^{NTK}(x)$ generalizes poorly. For $d=1$, the NTK $K(x,x')$ is given by
  \begin{equation}\label{ntk:L=1:d=1}
    K(x,x')= 2\left(1-\psi(x,x')/\pi\right)(x x'+1) +|x-x'| /\pi+1,
\end{equation}
where $\psi(x,x') = \arccos(\frac{xx'+1}{\sqrt{(x^2+1)(x'^2+1)}})\in[0,\frac{\pi}{4}]$.

We are interested in the behaviour of $f^{\NTK}_{t}$ when $t$ is sufficiently large, which represents overfitted neural networks. Given the specific kernel $K$, we can consider Kernel Ridgeless Regression, which is presented as

\begin{equation}\label{eq:ridgeless}
    f(x) = K(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}.
\end{equation}

 In the absence of explicit regularization, Kernel Ridgeless Regression with nonlinear kernels has the potential to fit the data points perfectly. The kernel can be chosen like RBF kernel or polynomial kernel. Compared with Equation \eqref{ntk:solution} and \eqref{eq:ridgeless}, as $t\to\infty$, Equation \eqref{ntk:solution} becomes Kernel Ridgeless Regression with NTK. Thus, we will discuss the behaviour of $f^{\NTK}_{\infty}(x) = K(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}$ in this section, which represents overfitted neural networks that can interpolate the data points.

To be more concrete, we consider the equally-distanced one dimensional data $\{\bm{X},\bm{y}\}=\{(x_{i},y_{i}) \mid x_{i}=\frac{i-1}{n-1}, i \in [n]\}$ as an example. We will focus on the performance of $f^{\NTK}_{\infty}(x)$ on such data. Under the bounded input $x_i$, we can get the bounded $f^*(x_i)$. Let $y_{max} = \max_{i\in[n]} y_i$. we can have the upper bound of $y_{max}$ through the following lemma:
\begin{lemma}\label{lem:bound_y}
With the definition of Equation \eqref{equation:true_model}, with the probability at least $1-\frac{2}{n}$, we have 
\begin{equation}
    y_{max} \leq C\sqrt{\log(n)}
\end{equation}
 and for some constant $C$.
\end{lemma}


\subsection{Overfitted Neural Network can be approximated by the linear interpolation}\label{ntk:linear interpolation}

Let
\begin{align}
    f_{\LI}(x)=y_{i}+\frac{y_{i+1}-y_{i}}{x_{i+1}-x_{i}}(x-x_{i}), \mbox{ when } x\in [x_{i},x_{i+1}]
\end{align}
be the linear interpolation of these $n$ points. We can prove the following statement.
\begin{proposition}[Bounded second order derivative of overfitted NTK model]\label{prop:bound_second_derivative}
Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. With the probability in Lemma \ref{lem:bound_y}, the second order derivative of the overfitted NTK model with zero initialization $f^{\NTK}_{\infty}(x) =K(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}$ is bounded, i.e.,
\begin{align}
 \sup_{x\in (x_i,x_{i+1})}|K''(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}|\leq C\sqrt{\log(n)} 
\end{align}
 for $\forall i\in[n]$ and for some constant $C$.
\end{proposition}
\begin{remark}
If we assume all the labels $\bm{y}$ are bounded(e.g., classification problems), i.e., $|y_i|\leq C$, $ j\in[n]$, the upper bound of Proposition \ref{prop:bound_second_derivative} will be the constant instead of $C\sqrt{\log(n)}$. Proposition \ref{prop:bound_second_derivative} is infrequent in many kernels such as Gaussian kernel or Polynomial kernel. 
\end{remark}

Through Taylor expansion, this property can guarantee that the linear interpolation can approximate the model as $n$ is increasing. Thus, we have the following corollary:

\begin{corollary}
[Overfitted NTK model can be approximated by the linear interpolation]\label{LI}
Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. With the probability in Lemma \ref{lem:bound_y}, the overfitted NTK model with zero initialization $f^{\NTK}_{\infty}(x) =K(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}$ can be approximated by the linear interpolation, i.e.,
\begin{align}
 \sup_{x\in [0,1]}|f_{\infty}^{\NTK}(x)-f_{\LI}(x)|\leq C\sqrt{\log(n)} /(n-1)^{2}
\end{align}
 for some constant $C$.
\end{corollary}

\begin{remark}
 To best of our knowledge, it is the first time to show how wide neural networks interpolate on the data. Combined with Proposition \ref{prop: function closeness} and Proposition \ref{LI} , our theory shows that for overfitted neural networks, adding more parameters does not increase the model complexity but make the models more concise (experiment results shown in Figure \ref{fig:LI} (a)). That is the reason why overfitted neural networks does not affect too much by the overparameterization.
\end{remark}

 Different from RBF kernel (or high order polynomial kernel) ridgeless regression,  Figure \ref{fig:LI} (a) and (b) present that the interpolation ways of the overfitted NTK model $f^{NTK}_{\infty}(x)$ and wide neural network are nearly linear. Proposition \ref{LI} give the upper bound of the gap between the overfitted NTK model and the linear interpolation is $O(\frac{1}{n})$ while Figure \ref{fig:LI} (c) shows that the gap actually is exactly $O(\frac{1}{n})$. These experimental results are in line with the conclusions of Proposition \ref{prop: function closeness} and Proposition \ref{LI}.

\begin{figure}[htbp]\label{fig:LI}
    \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{NN_with_diff_m.png}
      \centerline{(a)}
  \end{minipage}%
  \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{LI_NTK_RBF.png}
      \centerline{(b)}
  \end{minipage}%
  \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{gap_between_NTK_LI.png}
      \centerline{(c)}
  \end{minipage}
  \caption{(a):The interpolation ways of one-hidden-layer neural networks with different width; (b):The interpolation ways of linear interpolation, $f^{NTK}_{\infty}(x)$ and RBF kernel regression with $\gamma=1$; (c): The gap between $f^{NTK}_{\infty}(x)$ and linear interpolation. The input of the training data is the equally-distanced one dimensional data $\{x_{i}=\frac{i-1}{n-1}, i \in [n]\}$. The label of the training data is randomly selected from $\{1,-1\}$, which does not contribute to the experiment result. The sample size $n=100,200,...,1000$}
\end{figure}



\subsection{Overfitted network generalizes poorly}

Proposition \ref{LI} implies that a lazy trained overfitted neural network can be approximated by the linear interpolation. On the other hand, it is well known that the linear interpolation does not generalize well. Thus, we have the following statement.

\begin{theorem}[Overfitted network generalizes poorly]\label{thm:bad_gen}
    Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. The error of the overfitted NTK model with zero initialization $f^{\NTK}_{\infty}(x) =K(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}$ is bounded away from zero, i.e.,
    \begin{equation}
        \Expc\lVert f^{\NTK}_{\infty}-f_{\star}\rVert^2 \geq  C
    \end{equation}
 for some constant $C$.
\end{theorem}
\begin{remark}
Theorem \ref{thm:bad_gen} is to give an example showing that the overfitted neural network can have bad generalization, which contradicts the observation  {\bf (S)}. Since the lower bound $C$ in Theorem \ref{thm:bad_gen} is related to the scale of the noise, we believe overfitted neural network can not generalize well in most cases unless the noise is small enough. Figure \ref{fig: NTK_poor_performance} gives more examples showing that, even for $d>1$, the generalization error of overfitted networks is bounded away from zero even if the sample size is increasing.
\end{remark}

%Talk about the result of high dimension through experiments

\begin{figure}[h]
\centering
\includegraphics[scale=0.5]{test_error_of_NTK.png}
\caption{The performance of overfitted neural networks on different dimensional data: The input $x \sim Unif(0,1)^d$ where $d=1,3,5$. The ground true function $f^*(x) = sin(\frac{\sum_{j=1}^{d}x_j}{\sqrt{d}})$ and $y=f^*(x)+0.1\epsilon$, where $\epsilon \sim N(0,1)$. The sample size of training data $n=100,200,...,1000$ and the number of testing data is $1000$ for all experiments.}
\label{fig: NTK_poor_performance}
\end{figure}





==> SNR.tex <==
%Define the asymtotical NTK function f
In this section, we will talk about the two reasons why the overfitted neural network can still generalize:

{\it $\bullet$ the smoothness of data associated with NTK is large;} 

{\it $\bullet$ the noise of data is small and 100\%-training-accuracy stopping time is a kind of implicit early stopping.} 

Here, we emphasize that the smoothness of data should be considered together with NTK. More specifically, we should consider the interpolation spaces of NTK.

\subsection{Smoothness of data associated with NTK}
%Definition of RKHS
In Section \ref{ntk:recollect}, we have defined the integral operator $T_K$ associated with NTK. Upon the definition of $T_K$, we can also define the power $s$ of $T_K$
\begin{equation}
    T_K^{s} = \sum_{j=0} \lambda_j^{s} \phi_{j}\otimes \phi_{j}
\end{equation}
and the interpolation spaces with the power $s\geq 0$ of $T_K$
\begin{equation}
    [\mathcal{H}_K]^s:=\left\{\sum_{j=0}^{\infty}c_j\phi_j \big| \sum_{j=0}^{\infty} \frac{c_j^2}{\lambda_j^s}<\infty \right\}.
\end{equation} 
Obviously, $[\mathcal{H}_K]^1\subseteq \mathcal{H}_K$. For a function $f\in\mathcal{H}_K$, if $f\in [\mathcal{H}_K]^s$, $s$ represents the smoothness with respect to NTK, which is also considered as the signal of the function associated with the kernel. We tend to believe that the ground true function $f^*$ of the image data(e.g. MNIST, Cifar-10) is super smooth with respect to NTK(or CNTK). 

The function with high smoothness can be easily fitted. For example, if the ground true function is the eigenfunction corresponding to the largest eigenvalue of NTK, i.e.,
\begin{equation}\label{eq:strong_signal_eq}
    f^*(x) = \phi_0(x),
\end{equation}
that means $s$ is infinite by definition and the ground true function is infinitely smooth. To simply this case, we assume the data has no noise, $Y_n=f^*(X_n)$. Let $x_i\in[0,1]$ and $X_n=[x_1,...,x_n]$. $\frac{1}{n}K=P D P^{\tau}$, where $P$ is an orthogonal matrix, $P=[p_1,...,p_n]$ and $p_i, i\in [n]$ is the eigenvector.  $D$ is the diagonal matrix, $D=\operatorname{diag}\{\hat{\lambda}_1,\dots,\hat{\lambda}_n\}$ and $\hat{\lambda}_1\geq \hat{\lambda}_2 \geq \dots \geq \hat{\lambda}_n$. From Equation \eqref{ntk:solution}, we have
\begin{equation}
    f_{t}^{\NTK}(X_n) = (I-e^{-\frac{t}{n}K})Y_n = P(I-e^{-tD})P^{\tau} Y_n.
\end{equation}

It is well-known that under mild conditions, the eigenvectors of the kernel matrix converge to the eigenfunctions of the kernel. By Theorem 2.1 in \cite{koltchinskii1998asymptotics}, we have 
\begin{equation}
    \frac{1}{\sqrt{n}}|p_i\phi_{0}(X_n)| \to \delta_{i,1},a.s.,
\end{equation}
where $\delta_{11}=1$ and $\delta_{i1}=0$ for $i\neq 1$. which means $\frac{1}{\sqrt{n}}P^{\tau} Y_n$ is close to $(1,0,\dots,0)^{\tau}$. Typically, the eigenvector corresponding to the largest eigenvalue of the kernel matrix also holds if $n$ is sufficient large, i.e.,
\begin{equation}
    \sqrt{n}p_1 \to \phi_0(X_n),
\end{equation}
Thus, it is easy to find that within the finite time $t$, we have 
\begin{equation}
    f_t^{\NTK}(X_n) \to Y_n.
\end{equation}

In other words, the training loss can be close to zero and the training accuracy is close to 100\%. Of course, the generalization is good enough because of the small noise.

More generally, if the ground true function is the linear combination of the first few eigenfunctions and the noise is small, it is still infinite smooth and easily fitted as the example above. 

However, if the ground true function is not in $\mathcal{H}_K$, even if the noise is small, the overfitted neural network can not generalize. For example, the overfitted neural network can not generalize on odd/even prediction. More specifically, the input $x\in N$ and the ground true function $f^*(x)=1$ if x is odd and 0 otherwise. In this case, $\sum_{j=0}^{\infty} \frac{c_j^2}{\lambda_j}$ is not bounded(the estimations of $c_j$ are shown in Figure \ref{fig:signal}). Thus, $f^*(x)$ is not in $\mathcal{H}_K$ and the overfitted neural network can not generalize even if the data has no noise.

\subsection{Noise of data}

In regression problems, the noise is defined as 
\begin{equation}
    \epsilon = y - f^*(x).
\end{equation}
In binary classification problems, the true label is defined as
\begin{equation}
    y_{true}=1_{f^*(x)>0.5}.
\end{equation}
The labels of data is possibly different from the true labels. Thus, there is also a gap between the labels $Y_n$ and the ground true function on training set $f^*(X_n)$ since $Y_n$ are discrete integers and $f^*(X_n)$ are continuous. This gap is also considered as the noise of data. If the noise does not affect the true label, we can consider the noise is small. For example, $f^*(x_1)=0.1$ and the label $y_1=0$ and $f^*(x_2)=0.9$ and the label $y_1=1$. These two data points has small noise since the gap does not affect the true labels of $f^*(x_1)$ and $f^*(x_2)$. 

In general, the epoch with the maximum accuracy on validation set or the long-time unchanged training loss is commonly chosen as the stopping time. In this case, early stopping is potentially used. If the neural network is trained until it reach 100\% training accuracy, we tend to believe the network violates the conditions of early stopping and can not have good performance on testing set. However, if the noise is small, 100\% training accuracy does not mean the sufficient small loss(like Figure \ref{fig: interpolation vs acc}). The neural network may have large training loss even if it reaches 100\% training accuracy, which means the training process is early stopped before the interpolation regime.

If the noise is large, the 100\%-training-accuracy neural network can not have good generalization. For example, if $f^*(x_3)=0.1$ but the label $y_3=1$, that means the noise affects the true label of $f^*(x_3)$, which is called the label corruption in previous works(\cite{zhang2016understanding}). From Figure \ref{fig: MLP_diff_noise_mse} and \ref{fig: Alexnet_cifar10_diff_noise_ce}, we can find that as the percentage of label corruption is increasing, the training time to 100\% training accuracy is increasing. Moreover, the generalization gap between '100\% training accuracy' and 'best generalization' becomes larger. In these cases, explicit early stopping(e.g. cross validation) is still significant to the generalization of the model.


==> draft.tex <==
Since $X$ is one dimensional data(i.e., $d=1$), there is a simple formula for the NTK $K_{1}(x,x^{\prime})$: 
\begin{align*}
    K_{1}(x,x^{\prime}) &= \frac{2}{\pi}(1-\psi(x,x^{\prime}))(1+xx^{\prime}) + \frac{1}{\pi}|x-x^{\prime}| +1\\
    &= G(x,x^{\prime}) + 2\Pi_1(x,x^{\prime})=2\Pi_0(x,x^{\prime})(1+xx') - G(x,x') +2,
\end{align*}
where $G(x,x^{\prime}) = 1-\frac{|x-x'|}{\pi}$. Since $K=G+2\Pi_{1}$ and $\Pi_{1}$ is semi-positive definite, we know that $\forall X=\{x_{1},...,x_{n}\}\subset [0,\pi]$,
  $\lambda_{\min}(K(\bm{X},\bm{X})) \geq \lambda_{\min} (G(\bm{X},\bm{X}))$.

  

==> explanation.12.7.save.tex <==
In this section, we provide an explanation to reconcile our theoretical results and the widely observed phenomenon that ``overfitted neural network generalizes well''(e.g., \cite{zhang2016understanding},\cite{belkin2019does},\cite{belkin2018understand}). 

To be precise, Zhang et al.  \cite{zhang2016understanding} claimed the following observations: 

1. neural networks can easily reach the perfect 100\% training accuracy;

2. early stopping can slightly improve generalization on ImageNet;

3. early stopping is not necessarily helpful on CIFAR10 and the neural network with 100\% training accuracy can generalize well on CIFAR10;

%4. the absence of all explicit/implicit regularization(including early stopping) does not imply poor generalization error.

Thus, we have the essential observations claimed in \cite{zhang2016understanding}:

\noindent {\bf (S*)} \quad \quad \quad ``
The occurrence of the observation {\bf (S)} depends on the dataset.''
%Whether neural networks with 100\% training accuracy can generalize well depends on the dataset

On the other hand, we have shown in Section \ref{sec:main_result} that the performance of a trained over-parameterized neural network depends on the time stopping the training process: i) if the training process stops at a properly chosen time, the resulting neural network can achieve the minimax rate; ii) if the training process stops when the loss is near zero (or overfitting the data), the resulting neural network can not generalize well.  The latter statement seems to contradict the observation {\bf (S)}.


First of all, we have to emphasize that a subtle difference between the zero training loss and zero training label error might be ignored since the loss of the epoch with zero training label error is too small compared with the loss in the beginning. However, the stopping rule that the training process stops till zero label error might happen much earlier than the stopping rule that the training process stops till the (near) zero loss. This difference can be easily seen from the following illustrative example. 

Given 4 training data points $\{(0,0),(\frac{1}{3},1),(\frac{2}{3},0), (1,1) \}$, we use gradient descent to train a one-hidden-layer neural network with squared loss and the width $m=1000$. We define that the neural network is in the interpolation regime if the training loss is equal to zero. Compared with the interpolation regime, the training process stops till zero label error stops earlier and the loss is still large. The function with zero training label error is also far different from the function in the interpolation regime. The numerical result is reported in figure \ref{fig: interpolation vs acc} .%{\color{red} some detailed description about your example.}


\begin{figure}[h]\label{figure:3}
	\centering
	\includegraphics[scale=0.4]{100accuracy_vs_interpolation}
	\caption{Overfitting vs. 100 \% label accuracy: The left figure presents the loss and the accuracy of 4 training data points. The right figure shows the function in the epoch with 100 \% label accuracy and in the interpolation regime.}
	\label{fig: interpolation vs acc}
\end{figure}



% However, we realize that it might be caused by the subtle difference between zero training label error and zero training loss. In other words, the training till zero training label error is actually stopped earlier than the time till interpolating the data. We present this subtle difference through the following illustrative example.


%Although we realize the stopping time with zero training label error can be an implicit early stopping, we find that the occurrence of this implicit early stopping depends on the scale of the noise(the fraction of label corruption). In other words, the signal strength of data plays a significant role in this case.

%On the one hand, the Proposition \ref{prop:early:stopping} suggests that the performance of resulting neural network depends on the stopping time, and a carefully chosen early stopping time (optimal stopping rule) will produce a neural network  achieving the minimax rate.
What Zhang et al. \cite{zhang2016understanding} observed is that by stopping the training process when the 100\% label accuracy is reached, the resulting neural network can generalize well. It might be true that this particular implicit early stopping rule is close to the optimal stopping rule stated in Proposition \ref{prop:early:stopping}. 

%However, this sounds too good to be true. 

%On the other hand, the figure \ref{fig: interpolation vs acc} suggests that there might be a non-ignorable difference between stopping at zero label error and stoping at (near) zero loss error. It is most likely that this difference leads the observation that `overfitted' neural network generalizes well. 


%Zhang et al. \cite{zhang2016understanding} observed the implicit early stopping strategy, stopping the training process when the 100\% label accuracy is reached, can generalize well. One may speculate that the implicit early stopping time is the optimal stopping time that appeared in Proposition \ref{prop:early:stopping}. However, this sounds too good to be true. In fact, Zhang et al. \cite{zhang2016understanding} have discussed the role of some explicit early stopping strategies in training neural networks. They observed that: 1. early stopping indeed makes generalization better on ImageNet, and 2. early stopping does not help much on CIFAR10. These observations made the effects of the implicit early stopping elusive. We can not simply claim that the implicit early-stopping strategy would produce a rate-optimal neural network.


As suggested by the observation {\bf (S*)}, we hypothesized that signal strength plays an indispensable role in the success of implicit early-stopping strategies. More precisely, when the signal strength is strong enough, the implicit early stopping strategy will produce a stopping time near the optimal stopping time $t_{\star}$; and when the signal strength deteriorates (e.g., after performing label corruption procedure), the implicit early stopping strategy will produce a stopping time far from the optimal stopping time $t_{\star}$. 

%Talk about what is the signal strength: Smoothness and the scale of noise
%We will talk about the two reasons why the overfitted neural network can still generalize:

Experiments from \cite{belkin2018understand} show that ``early stopping provides at most a minor improvement to classifier performance'' and MNIST labels are arguably close to a deterministic function of the features, as most (but not all) digit images are easily recognizable.

\begin{comment}
\subsection{Noise of data}

%Define the scale of noise
In Section \ref{intro}, we assume the noise $\epsilon\sim N(0,\sigma)$, which is too good to be true in real cases. Nevertheless, we can still believe there is a ground-true function $f_{\star}(\bm{x})$ behind the data. Thus, we can define the gap between the label and the ground-true function as noise, i.e.,
\begin{equation}
    \epsilon = y - f_{\star}(x).
\end{equation}
In binary classification problems, the true label can be defined as
\begin{equation}
    y_{\text{true}}=\bm{1}_{f_{\star}(x)>0.5}.
\end{equation}
The labels of data $y$ are possibly different from the true labels $y_{\text{true}}$. Since the ground-true function is unknown and we actually care about the true label, we can define the small noise as followed:
\begin{definition}
    The noise of the data point $x,y$ is small if 
    \begin{equation}
        y=y_{\text{true}}
    \end{equation}
\end{definition}

For example, $f_{\star}(x_1)=0.1$ and the label $y_1=0$ and $f_{\star}(x_2)=0.6$ and the label $y_1=1$. These two data points have small noise since the gap does not affect the true labels of $f_{\star}(x_1)$ and $f_{\star}(x_2)$ even if the square losses of these two points are different. However, if the noise affects the true label, that means label corruption happens. For example, if $f_{\star}(x_3)=0.1$ but the label $y_3=1$, that means the noise affects the true label of $f_{\star}(x_3)$.

In general, the epoch with the maximum accuracy on the validation set or the long-time unchanged training loss is commonly chosen as the stopping time. In this case, early stopping is potentially used. If the neural network is trained until it reaches 100\% training accuracy, we tend to believe the network violates the conditions of early stopping and can not have a good performance on the testing set. However, even if the noise is small, 100\% training accuracy does not mean a sufficient small loss. The neural network may have a large training loss even if it reaches 100\% training accuracy, which means the training process is early stopped before the interpolation regime.

If the noise is large, the 100\%-training-accuracy neural network can not have good generalization. From Figure \ref{fig: MLP_diff_noise_mse} and \ref{fig: Alexnet_cifar10_diff_noise_ce}, we can find that as the percentage of label corruption is increasing, the training time to 100\% training accuracy is increasing. Moreover, the generalization gap between `100\% training accuracy' and `best generalization' becomes larger. In these cases, explicit early stopping(e.g. cross validation) is still significant to the generalization of the model.

In summary, we finally filled the last piece of the jigsaw in reconciling the controversial observation (S) and the bias-variance trade-off doctrine in classical statistical learning theory.

\end{comment}


==> intro.save.12.4.tex <==
% NN is awesome in practice.
Deep neural networks have been successfully applied in various fields such as image analysis, natural language processing, protein structure prediction, etc.\cite{krizhevsky2012imagenet, devlin2019bert, jumper2021highly}. Since the number of parameters appeared in the deep neural network is often ten times or hundred times larger than the sample size of data, the successes of neural networks have challenged the traditional bias variances trade-off principle, one of the primary doctrines in the classical statistical learning theories \cite{vapnik1995nature}.

For example, many influential experiments in Zhang et al.(2016) \cite{zhang2016understanding} suggested that if one trains a neural network till it is overfitting the data, the resulting network can still generalize well. This observation,

\noindent {\bf (S)} \quad \quad   \textit{`Neural networks can generalize well even with the 100\% training accuracy,'} 

\noindent actually reshaped the landscape of the research in understanding neural networks. It seems that neural networks can exhibit a remarkably small difference between the training and the test performance and the traditional approaches fail to explain why neural networks can generalize well in practice. 

% NN is minimax optimal ERM existence
% \cite{kohler2005adaptive}(Hölder class), \cite{imaizumi2019deep}(piecewise Hölder class),  \cite{suzuki2019adaptivity}(Besov class and its variant), \cite{hayakawa2020minimax}(class with discontinuity and sparsity) and \cite{suzuki2021deep}(anisotropic Besov class), etc. 
% Based on approximation theory \cite{pinkus1999approximation}

% why ERM
%Several groups of statisticians tried to explain the generalization ability of neural network from various carefully designed nonprametric regression frameworks. 
%For example,  \cite{bauer2019deep} proved the minimax rate optimality of neural networks with activation function $\sigma(\cdot)$ satisfying $\lim_{z\to-\infty}\sigma(z)=0$ and $\lim_{z\to\infty}\sigma(z)=1$ when the regression function belongs to a class of functions consisting of a composite of Hölder smooth functions; \cite{schmidt-hieber2020nonparametric} further established similar results for ReLU based on approximation theory from \cite{yarotsky2017error}; \cite{suzuki2019adaptivity} then extended the result to regression functions in Besov space and its variants. 
%Most of these works \cite{kohler2005adaptive, petersen2018optimal, schmidt-hieber2020nonparametric, bauer2019deep, imaizumi2019deep, suzuki2019adaptivity, hayakawa2020minimax, suzuki2021deep,kim2021fast} first proposed  some unusual assumptions on the class of the underlying ground truth;  they then showed that the empirical risk minimizer (ERM) of some carefully choosed loss function over neural networks  can achieve the theoretical optimal rate over the prescribed class of models.

Typically, once the structure of the neural networks is given, one tries to determine the specific parameters under the guidance of the training data. Minimizing the training loss is a classical standard. Hence, many researchers have investigated the generalization performance of neural networks from the perspective of the ERM(empirical risk minimizer). Overall, a line work has shown that with appropriate assumptions on the underlying ground truth, there exists some ERMs among the hypothesis class of the neural networks that can be endowed with the minimax rate optimality both in regression \cite{kohler2005adaptive, petersen2018optimal, schmidt-hieber2020nonparametric, bauer2019deep, imaizumi2019deep, suzuki2019adaptivity, hayakawa2020minimax, suzuki2021deep} and classification \cite{kim2021fast} tasks. To name a few, \cite{bauer2019deep} proved the minimax rate optimality of neural networks with activation function $\sigma(\cdot)$ satisfying $\lim_{z\to-\infty}\sigma(z)=0$ and $\lim_{z\to\infty}\sigma(z)=1$ when the regression function is a composite of Hölder smooth functions, \cite{schmidt-hieber2020nonparametric} further established similar results for ReLU based on approximation theory from \cite{yarotsky2017error}, \cite{suzuki2019adaptivity} then extended the result to regression functions in Besov space and its variant. However, the restrictions on parameters of neural networks from these works like boundedness and sparsity may not be realistic. Most importantly, these theoretical results have no algorithmic guarantees. Thus, the generalization performance of ERMs found by algorithms in practice, especially gradient descent is of great interest.


% NN Approximation
Analysis of the original neural network trained by gradient descent(GD) or stochastic gradient descent(SGD) is a real challenge. Many works tried to first understand the neural networks with a very large width, as neural networks implemented in practice are indeed over-parameterized. There is a line of work taking a mean-field analysis \cite{mei2018mean, mei2019mean}. \cite{mei2018mean} has developed an analysis of SGD dynamics that connects to the theory of universal approximation. The analysis shows that for a large width, the empirical distribution of the parameters can be approximated by a probability distribution, which evolves according to the width-independent partial differential equation, referred to as distributional dynamics. Another line of work is based on the phenomenon that the parameters of over-parameterized neural networks hardly vary when training loss could converge exponentially fast to zero, which is called as ``lazy training'' phenomenon \cite{chizat2019lazy}. \cite{jacot2018neural} gave a theoretical proof of such a phenomenon, showing that the evolution of neural networks with the bounded-second-derivative activation function can also be described by a fixed limiting kernel, called Neural Tangent Kernel(NTK). \cite{du2018gradient} further proved that over-parameterized two-layers ReLU networks have the same property. However, neither shows uniform approximation for overparameterized neural networks, which is the key to the approximation for the generalization ability of overparameterized neural networks. 


% NN can find by global minimum by GD 
In the ``lazy training'' regime, overparameterized neural networks trained by gradient descent can achieve zero training loss\cite{li2018learning, du2018gradient, du2019gradient, allen2019convergence}. Their analysis relies on the particular structure of the Gram matrix induced by the neural network architecture. In the ``lazy training" regime, the Gram matrix is stable throughout the training process and the stability of the Gram matrix guarantees the exponential decrease of the loss. However, the generalization ability of the minimizers with zero training loss has not been discussed in these works. Or the good generalization of these minimizers only holds under the noiseless assumption. 


% What we do
Though the above theories have been proposed to explain these observations and lots of experiments have been carried on to justify these theories, they are still far from satisfying theories. In this paper, we provide an explanation that might reconcile the bias-variance trade-off doctrine and the statement (S). We first show that the gradient flow of the over-parameterized two-layers ReLU neural networks uniformly converges to the gradient flow of the corresponding RKHS associated with the NTK as the width of the neural networks is increasing in Section \ref{subsec:ntk:approx}. With the assistance of the uniform convergence, we then show in Section \ref{subsec:generalization} through a one-dimensional example that neural networks with early stopping are minimax rate optimal and overfitted neural networks can not generalize well. We recognize that there is a subtle difference between training the neural network till the 100\% training accuracy of the labels and till the zero training error of the loss function. This leads us to recognize an implicit early-stopping phenomenon in the training processes and its role in explaining the generalization ability of the resulting neural network. Finally, we reveal the role played by signal strength in the statement (S).


\subsection{Contributions} 

In this paper, we focus on the training process of the over-parameterized two-layers neural network in the so-called ``lazy training'' regime. That is, the width of the neural networks is sufficiently large so that the dynamics of the training process can be approximated well by the dynamics of the corresponding NTK.

{\it $\bullet$ Properties of NTK.} 
We first show that NTK is strictly positive definite on $\mathbb{R}^{d}$, which fills a long-standing gap in the literature. We then provide the seemingly sharpest bounds on the minimum eigenvalue of gram matrix $(K(\bm{x}_{i},\bm{x}_{j}))_{1\leq i,j\leq n}$ for one-dimensional data. Since most of the existing studies on the spectral properties of NTK are focused on those defined on a sphere $\mathbb{S}^{d-1}$, we are lacking of basic knowledge about the spectral properties of the NTK on $\mathbb{R}^{d}$. We show the decay rate of the eigenvalues on $[0,1]\in \mathbb{R}$. Our work shed light on the possibility of obtaining more explicit knowledge about the spectral properties of NTK on $\mathbb{R}^{d}$. This would be of great interest to researchers.

{\it $\bullet$ Uniform NTK approximation for over-parameterized neural networks.} Many works have claimed that wide neural networks can be approximated by NTK. However, they only prove the point-wise kernel approximation and function approximation. Here we give a refined analysis to show that the over-parameterized two-layers ReLU neural networks can be approximated by NTK uniformly. Thus the generalization performance of the neural networks can be represented by NTK safely.

{\it $\bullet$ Generalization performance of neural networks on $\mathbb{R}$.}
With the decay rate of the eigenvalue of the NTK, we prove that over-parameterized neural networks trained by GD achieves the minimax-optimal rate $n^{-2/3}$. Moreover, we show that if one trains a over-parameterized two-layers neural network till it over-fits the equally-distanced one-dimensional data, the resulting neural network is essentially a linear interpolation. Thus, an over-fitted neural network can not generalize well. Though this claim is simple, it is the first time that we have a concrete understanding of what an over-fitted neural network looks like.
%{\it $\bullet$ Neural networks are minimax optimal with early stopping.}
%With the decay rate of the eigenvalue of the NTK, we prove that overparameterized neural network trained by GD achieves the minimax-optimal convergence rate $n^{-2/3}$. 

%{\it $\bullet$ Overfitted neural network can not generalize well.} 
%With the popularity of this observation {\bf (S)} is reported in \cite{zhang2016understanding}, many researchers try to show that overfitted neural models/neural networks can generalize well(e.g., \cite{belkin2019does},\cite{liang2020just}). However, we showed that if one trains a wide 1-hidden layer neural network till it overfits the equally-distanced one-dimensional data, the resulting neural network is essentially a linear interpolation. Thus, an overfitted neural network can not generalize well. Though this claim is simple, it is the first time that we have a concrete understanding of what an overfitted neural network looks like.

{\it $\bullet$ Why over-fitted neural networks can generalize: (implicit) early stopping.} Though lots of experiments have reported that over-fitted neural networks can generalize, a subtle difference between 100\% training accuracy of labels and zero training loss might be ignored. This difference actually leads the training process being stopped earlier than the time needed to over-fit the data. We refer to this fact as implicit early stopping. However, we find that the occurrence of this implicit early stopping depends on the signal strength of the data. We further illustrate through several experiments that signal strength explains when the implicit early stopping strategy results a neural network achieving the optimal generalization ability.

\subsection{Related works}
\subsubsection*{NTK properties on $S^{d-1}$} To the best of our knowledge, most works studying the generalization ability of neural networks are either working on $\mathbb{S}^{d-1}$ or assuming that $\lambda_{\min}$, the minimum eigenvalue of the Gram matrix $(K(\bm{x}_{i},\bm{x}_{j}))_{1\leq i,j\leq n}$ associated to the NTK $K$ and the data set $\{\bm{x}_{i}, i=1,\cdots,n\}$, is positive (e.g., \cite{du2018gradient, hu2021regularization}). The strictly positive definiteness of NTK on $\mathbb{S}^{d-1}$ is proved by \cite{jacot2018neural}, including ReLU NTK. For the decay rate of the eigenvalue of ReLU NTK on $\mathbb{S}^{d-1}$, it can be used to analyze the reproducing kernel Hilbert space of NTK. Many previous works \cite{bietti2019inductive, bietti2020deep, cao2019towards} have shown the decay rate of the eigenvalues $\lambda_j$ of NTK on $\mathbb{S}^{d-1}$. For the minimum eigenvalue of the $n\times n$ kernel matrix, it can indicate the convergent rate of the over-parameterized neural network. \cite{nguyen2021tight} gives a bound of the minimum eigenvalue related to the dimension of inputs $d$ instead of sample size $n$, which can not be used when $n$ is larger compared with $d$. Many results of NTK properties are solved on $\mathbb{S}^{d}$. But the works on $\mathbb{R}^d$ are still waiting for solutions.

% \cite{hu2021regularization}, \cite{suh2021non} can reach the minimax rate by $l_2$-regularized GD. 
\subsubsection*{The generalization performance of neural networks trained by GD} Several works study the generalization ability of neural networks with GD. Specifically, with the result of spectral properties of NTK on $\mathbb{S}^{d-1}$ mentioned above. \cite{hu2021regularization} claimed that if the ground true function is from the RKHS with NTK, an over-parameterized two-layers neural network trained by $l_2$-regularized GD can reach the minimax optimal rate. \cite{suh2022nonparametric} further showed the same generalization property of deep neural networks. For vanilla GD, without early stopping, \cite{hu2021regularization} and \cite{suh2022nonparametric} claimed that over-trained neural networks can not generalize well, i.e., the generalization error is bounded away from zero as the sample size goes to infinity. However, their claims rely on an unproved result (the second statement of the Corollary 3 in \cite{raskutti2014early}) essentially.

%Explanation
\subsubsection*{Explanations of why over-fitted neural networks can generalize well} 
Although some theoretical results claimed that over-fitted neural networks can not generalize well, other papers still try to show that over-fitted models/neural networks can generalize well(e.g., \cite{belkin2019does, liang2020just}). In particular, \cite{belkin2019does} exhibited the Nadaraya-Watson estimator that interpolates the data, yet achieves minimax optimal rates of convergence. However, this kind of interpolation is far different from the interpolation that neural networks do. \cite{liang2020just} presented that Kernel ``Ridgeless'' Regression with non-linear kernels, that perfectly fits the training data, can still generalize well on test data. But such generalization ability needs high dimensional assumption: the ratio of dimension to sample size should be constant.



%\subsection{Outline}
%The uniform NTK approximation for wide neural networks and the strictly positive definiteness of NTK on $\mathbb{R}^d$ are presented in Section \ref{ntk:recollect}. In the meantime, a sharped lower bound on the minimum eigenvalue of the gram matrix $(K(\bm{x}_i,\bm{x}_j))_{1\leq i\leq j\leq n}$ is given as an example for one-dimensional data. In Section \ref{sec:main_result}, we give an example showing that the overfitted neural network can not generalize well. Section \ref{sec:early_stopping} shows that wide neural networks can reach minimax optimal rate with early stopping and the fact that 100\%-training-accuracy stopping policy is a kind of implicit early stopping depending on the signal strength of data. Several experiments are illustrated in Section \ref{sec:experments}.

\vspace{3mm}
\subsection{Preliminary}

Let's consider $n$ i.i.d. samples $\{(\boldsymbol{x}_i,y_i)\}_{i=1}^{n}$ from an unknown distribution $\mu_{\mathcal{X}}\times\mu_{\mathcal{Y}}$ supported on $\mathcal{X}\times \mathcal{Y}$ where $\mathcal{X}\in\mathbb{R}^d$ and $\mathcal{Y}\in\mathbb{R}$. 

The samples are from the model 
\begin{equation}\label{equation:true_model}
    y=f_{\star}(\boldsymbol{x})+\varepsilon, \quad \varepsilon\sim N(0,\sigma^{2}).
\end{equation}
where $f_{\star}$ is an unknown regression function and $\varepsilon$ is independent random variables. Based on these $n$ samples, we are interested in finding a function $\hat{f}_{n}$ such that risk
\begin{equation}
    \poprisk(\hat{f}_{n})=\Expc_{(\bm{x},y)}\left[(\hat{f}_{n}(\bm{x})-y)^2\right]
\end{equation}
is as small as possible. The best possible one can get is by choosing $\hat{f}$ to be $f_{\star}=\Expc(y\mid \bm{x})$. From now on, we use excess risk 
\begin{equation}\label{eq:excrisk}
    \excrisk(\hat{f}_{n})=\poprisk(\hat{f}_{n})-\poprisk(f_{\star})=\int_{\mathcal{X}}(\hat{f}_{n}(\bm{x})-f_{\star}(\bm{x})^{2}) \dx \mu_{\mathcal{X}}(\bm{x})
\end{equation}
to evaluate the generalization performance.

To better estimate the regression function $f_{\star}(\boldsymbol{x})$, we can consider the machinery of reproducing kernel Hilbert spaces(RKHS). Let's consider a Hilbert space $\mathcal{H}\subset L_{\mu_{\mathcal{X}}}^{2}$ associated with an inner product $\langle \cdot, \cdot\rangle_{\mathcal{H}}$. If there exists a continuous, symmetric and positive definite function $K:\mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}$ such that $\boldsymbol{x}\in \mathbb{R}^d$, $K(\boldsymbol{x},\cdot)\in \mathcal{H}$ and for all $f\in\mathcal{H}$, $f(\boldsymbol{x}) = \langle f, K(\boldsymbol{x},\cdot) \rangle_{\mathcal{H}}$, then $\mathcal{H}$ is an RKHS. We can denote $\mathcal{H}_K$ as an RKHS associated with the kernel $K$.

The Mercer's decomposition theorem asserts that there exist $\phi_{0}(\boldsymbol{x}), \phi_{1}(\boldsymbol{x}),\phi_{2}(\boldsymbol{x}),\cdots \in L_{\mu_{\mathcal{X}}}^{2}(\mathcal{X})$ such that $\left<\phi_{i},\phi_{j}\right>_{L_{\mu_{\mathcal{X}}}^{2}}=\delta_{ij}$ and 
 \begin{align}
K(\boldsymbol{x},\boldsymbol{x}')=\sum_{j=0}^{\infty}\lambda_{j}\phi_{j}(\boldsymbol{x})\phi_{j}(\boldsymbol{x}'),\quad   j=0,1,2,\cdots,
 \end{align}
where $\lambda_0\geq \lambda_1,\dots,\geq 0$. We also refer to the $\{\lambda_{j},j=0,1,2,\cdots\}$ as the eigenvalues and $\phi_0,\phi_1,\dots$ are the eigenfunctions associated to the kernel $K$. At the same time, a integral operator $T_{K}:L_{\mu_{\mathcal{X}}}^{2} \to L_{\mu_{\mathcal{X}}}^{2} $ associated with $K$ can be defined as 
\begin{equation}
    (T_K f)(\boldsymbol{x}) = \int_{\mathcal{X}} K(\boldsymbol{x},\boldsymbol{x}') f(\boldsymbol{x}') d\mu_{\mathcal{X}}(\boldsymbol{x}), \quad \forall f \in L_{\mu_{\mathcal{X}}}^{2} 
\end{equation}
and we have the spectral decomposition of $T_K$:
\begin{equation}
    T_K=\sum_{j=0}^{\infty} \lambda_{j}\phi_j \otimes \phi_j
\end{equation}
With the eigenvalues and the eigenfunctions associated to the kernel $K$, $\mathcal{H}_K$ can be formulated as 
\begin{equation}
    \mathcal{H}_K = \left\{f=\sum_{j=0}^{\infty} c_j\lambda_j^{\frac{1}{2}} \phi_j ~\middle|~ \sum_{j=0}^{\infty}c_j^2 <\infty \right\}.
\end{equation}

% To make this problem solvable, we need some mild assumptions:
% \begin{assumption}
%     Each dimension of $\boldsymbol{x}$ is bounded by $B<\infty$. or $\lVert\bm{x}\rVert_2 \leq B$
% \end{assumption}













==> main_result.save.12.14.tex <==
To simplify the mathematical argument, we consider the gradient flow instead of the gradient descent in analyzing  the training process of neural networks. When view the loss function $\hat{\mathcal{L}}_{n}$ as a function defined on the parameter space $\Theta$, it induced a gradient flow in $\Theta$ given by
\begin{equation}\label{nn:theta:flow}
\begin{aligned}
      \dot{\bm{\theta}}(t) &=\frac{\dx}{\dx t}\bm{\theta}(t)=-\nabla_{\bm{\theta}}\emprisk(f_{\bm{\theta}})= - \frac{1}{n}\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})\tran (f_{\bm{\theta}(t)}(\bm{X})-\bm{y})
\end{aligned}
\end{equation}
where we emphasized that $\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})$ is an $n\times ((d+2)m+1)$ matrix.
When view the loss function $\hat{\mathcal{L}}_{n}$ as a function defined on the network space $\mathcal{F}^{m}$, it induced a gradient flow in $\mathcal{F}^{m}$ given by
\begin{equation}\label{nn:f:flow}
\begin{aligned} 
\dot{f}_{\bm{\theta}(t)}(\bm{x}) &=\frac{\dx }{\dx t}f_{\bm{\theta}(t)}(\bm{x})=\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{x})\dot{\bm{\theta}}(t)= -\frac{1}{n} K_{\bm{\theta}(t)}(\bm{x},\bm{X}) (f_{\bm{\theta}(t)}(\bm{X})-\bm{y}),
\end{aligned}
\end{equation}
where we emphasize that $K_{\bm{\theta}(t)}(\bm{x},\bm{X}) =\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{x}) \nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})\tran$ is a $1\times n$ vector. We further introduce a time-varying kernel function
\begin{align*}
K_{\bm{\theta}(t)}(\bm{x},\bm{y})=\nabla_{\bm{\theta}}f_{\bm{\theta}(t)}(\bm{x})\nabla_{\bm{\theta}}f_{\bm{\theta}(t)}(\bm{y}).
\end{align*}
To avoid potential confusion with the time-invariant neural tangent kernel,  we refer to this time-varing kernel  $K_{\bm{\theta}(t)}$ as the neural network kernel.

It is clear from the gradient flow Equations \eqref{nn:theta:flow} and \eqref{nn:f:flow} that the training process of neural network  is  determined by the initialization of $\bm{\theta}(0)$.
% ( and hence the $f_{\bm{\theta}(0)}(\bm{x})$). 
Since the $\bm{\theta}(0)$ is initialized randomly, the initial neural network $f_{\bm{\theta}(0)}(\bm{x})$ as well.  To avoid unnecessary digression, we adopt a special initialization widely used in literature so that $f_{\bm{\theta}(0)}(\bm{x})=0$. ({\color{red}citation}\cite{chizat2019lazy, hu2019simple})
%: we replicating a network with the same values on the first layer and opposite signs on the top layer at initialization and the bias term on the top layer is set as zero. 
More precisely, for a one-hidden layer neural network with width $2m$, we assume that $a_{r}(0),\bm{w}_{r,j}(0),b_{r}(0), \sim \mathcal{N}(0,1)$ for $r\in [m]$, $j\in [d]$, $a_{r+m}(0)=a_{r}(0)$, $\bm{w}_{r+m,j}(0)=\bm{w}_{r,j}(0)$, $b_{r+m}(0)=b_{r}(0)$ and $b =0$. 

Since it is hard to find an explicit solution of the highly non-linear equations \eqref{nn:theta:flow} and  \eqref{nn:f:flow} , researchers looked for approximated solutions characterizing the asymptotic behavior of the exact solution of these equations (see e.g.,\cite{mei2019mean, karakida2019universal, sirignano2022mean, eldan2021non}).
When the width $m\rightarrow\infty$,  
Jacot et al\cite{jacot2018neural} observed that for any $t\in \mathbb{R}_{\geq 0}$, $\bm{x},\bm{x}'\in \mathbb{R}^{d}$, one has 
\begin{align}
    K_{\bm{\theta}(t)}(\bm{x},\bm{x}')\xrightarrow{m\rightarrow \infty} K_d(\bm{x},\bm{x}')
\end{align}
where $K_d$ is a time-independent kernel defined on $\mathbb{R}^d$. This time-independent kernel, now often referred to as the neural tangent kernel (NTK), offered us a simplified version of the equations \eqref{nn:theta:flow} and \eqref{nn:f:flow}:
\begin{equation}\label{ntk:f:flow}
    \begin{aligned}
    \dot{f}^{\NTK}_{t}(\bm{x})=\frac{\dx}{\dx t}f^{\NTK}_{t}(\bm{x})=-\frac{1}{n}K_d(\bm{x},\bm{X})(f^{\NTK}_{t}(\bm{X})-\bm{y})
    \end{aligned}
\end{equation}
where  $K_d(\bm{x},\bm{X}) = (K_d(\bm{x},\bm{x}_1),\dots,K_d(\bm{x},\bm{x}_n))\in \mathbb{R}^{1\times n}$.
This equation is defined on the space $\mathcal{F}$, the RKHS associated to the kernel $K_{d}$. 
We referred to this equation \eqref{ntk:f:flow} as the gradient flow associated to the kernel regression with respect to the kernel $K_{d}$. 
Similar to the neural network function, we assume that the initial function $f^{\NTK}_{0}(\bm{x})=0$. 


Though it is hard to solve the equations \eqref{nn:theta:flow} and \eqref{nn:f:flow} directly,   the equation \eqref{ntk:f:flow}  can be solved explicitly:
\begin{equation}\label{ntk:solution}
    f_t^{\NTK}(\bm{x})=K_d(\bm{x},\bm{X})K_d(\bm{X},\bm{X})^{-1}(\bm{I}-e^{-\frac{1}{n}K_d(\bm{X},\bm{X})t})\bm{y}.
\end{equation}
Researchers believed that the solution $f^{m}_{\bm{\theta}(t)}$ can be well approximated by $f^{\NTK}_{t}$ when $m$ is sufficiently large and proved that for any $t\geq 0$, $\bm{x}\in \mathbb{R}^{d}$, one has the point-wise convergence(see e.g., {\color{red} citation\cite{vyas2022limitations, arora2019exact, arora2019fine, hu2021regularization, suh2022nonparametric}}, \cite{du2018gradient, du2019gradient, arora2019exact, lee2019wide}):
\begin{align}\label{eq:solution:convergence}
f^{m}_{\bm{\theta}(t)}(\bm{x}) \xrightarrow{m\rightarrow \infty} f_{t}^{\NTK}(\bm{x})
\end{align} 
One of our main technical contributions is that the above convergence is uniformly with respect to all $t\geq 0$ and  $\bm{x}\in \mathbb{R}^{d}$.

%However,  This simplifies the problem substantially, as we can solve the equation \eqref{ntk:f:flow} explicitly: 

%The uniform approximation between $f^{\NTK}_{t}(\bm{x})$ and $f_{\bm{\theta}(t)}$ will be presented in the next subsection.

\subsection{The excess risk $\mathcal{E}(f^{m}_{\bm{\theta}(t)})$ converges to  the excess risk $\mathcal{E}(f^{\NTK}_{t})$   } \label{subsec:ntk:approx}

% One may naturally expect that the solution $f_{\bm{\theta}(t)}$ of the equation \eqref{nn:f:flow} and the solution $f^{\NTK}_{t}$ of the equation \eqref{ntk:f:flow} should behave in a similar way for sufficiently large $m$.  
% Furthermore, when $m$ is sufficiently large, 
% some researchers often referred to the flow $f_{\bm{\theta}(t)}$ as the lazy trained neural network, for 
% the movement of $\bm{\theta}(t)$ is ignorable in this scenario (e.g., \cite{lee2019wide},\cite{du2018gradient},\cite{jacot2018neural}).
% These statements have been justified in a sequence of works from various groups of researchers (see e.g., \cite{jacot2018neural},\cite{arora2019exact},\cite{lee2019wide}). 

% #comparisons with other similar work

% We are aware that \cite{hu2021regularization}, \cite{suh2022nonparametric} have shown that the generalization error of the neural network trained for too long is bounded away from zero. However, it is worth noting that both of their results need NTK regression as an intermediate term. Then it is necessary to prove that the generalization error of the neural network could be approximated by that of NTK regression.

% why uniform NTK approximation is important

%Since the seminal work \cite{jacot2018neural} brought up the concept of the NTK, many works have been trying to understand the generalization performance of neural networks based on the NTK \cite{vyas2022limitations, arora2019exact, arora2019fine, hu2021regularization, suh2022nonparametric}. 
In this subsection, we show  in the following Theorem \ref{thm:risk:approx} that the excess risk of the very wide two-layers ReLU neural networks $f_{\bm{\theta}(t)}^{m}$ could be well arppoximated by the excess risk of $f_{t}^{\NTK}$. 
% and the precise argument is established in Theorem \ref{thm:risk:approx}, paving the way for the discussion about generalization performance of neural networks in Section \ref{subsec:generalization}. 

% With Theorem \ref{thm:risk:approx}, using NTK regression as a substitute to investigate the generalization performance of the over-parameterized two-layers ReLU neural network is rigorously valid. 

% In the following Section \ref{subsec:generalization}, the generalization performance of the fully trained overparameterized two-layers ReLU neural networks could be understood with the help of NTK regression in a carefree way.

% To the best of our knowledge, we give the first concrete result on that the generalization error of the fully trained two-layers ReLU neural networks could be represented by NTK regression, which is our Theorem \ref{thm:risk:approx}.

\begin{theorem}\label{thm:risk:approx}
    Given the training data, for all $t\geq 0$, if the width $m$ of the two-layers ReLU neural network is sufficiently large, then
    \begin{equation*}
        |\excrisk(f_{\bm{\theta}(t)})-\excrisk(f_{t}^{\NTK})|=o_{m}(1)
    \end{equation*}
    holds with probability converging to one 
    %over initialization 
    as the width $m$ goes to infinity. 
\end{theorem}
{\color{red}
\begin{proof}
   It is easy to see that $\excrisk(f_{\bm{\theta}(t)})-\excrisk(f_{t}^{\NTK})$ could be controlled by upper bounding   $\int_{\mathcal{X}}(f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x}))^{2}\dx\mu_{\mathcal{X}}(\bm{x})$ and $\int_{\mathcal{X}}(f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x}))(f_{t}^{\NTK}(\bm{x})-f_{\star}(\bm{x}))\dx \mu_{\mathcal{X}}(\bm{x})$. The term $\sup_{\bm{x}}|f_{t}^{\NTK}(\bm{x})-f_{\star}(\bm{x})|$ could be bounded by arguing that $f_{t}^{\NTK}$ and $f_{\star}$ are both continuous over the compact set $\mathcal{X}$. Thus
    \begin{equation*}
        |\excrisk(f_{\bm{\theta}(t)})-\excrisk(f_{t}^{\NTK})|=O(\sup_{\bm{x}}|f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})|),
    \end{equation*}
    indicating the uniform approximation of $f_{t}^{\NTK}$ to $f_{\bm{\theta}(t)}$, i.e., $\sup_{\bm{x}}|f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})|$ lies at the heart of the proof of Theorem \ref{thm:risk:approx}, which is provided in Proposition \ref{prop:funct:approx} below.
\end{proof}
}

% to prove this theorem, emphasize the importance of uniform convergence.

% A closer look at \eqref{eq:excrisk} suggests , since the generalization is related to all possible $\bm{x}$ drawn from $\mu_{X}$.

\begin{proposition}\label{prop:funct:approx}
    Given the training data, if the width $m$ of the two-layers ReLU neural network is sufficiently large, then for all $t\geq 0$, 
    \begin{equation*}
        \sup_{\bm{x}}| f^{m}_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})|=o_{m}(1)
    \end{equation*}
    holds with probability converging to one over initialization as the width $m$ goes to infinity.
\end{proposition}

% Check
% \begin{itemize}
%     \item $\alpha<1/2$
%     \item $1-\gamma<\beta/2$
%     \item $\gamma>\max\{1-\alpha,\delta\}$
%     \item $\beta>\alpha$
% \end{itemize}

It is clear in the proof of Theorem \ref{thm:risk:approx} that the neural network $f_{\bm{\theta}(t)}^{m}(\bm{x})$ converges uniformly to the function $f_{t}^{\NTK}(\bm{x})$  with high probability as $m\rightarrow\infty$ is indispensable. The existing results
    %Proposition \ref{prop:funct:approx} shows the difference between $f_{\bm{\theta}(t)}(\bm{x})$ and $f_{t}^{\NTK}(\bm{x})$ over all $\bm{x}$ can be controlled uniformly with high probability by the width $m$, 
  by \cite{lee2019wide, arora2019exact} only showed that for any fixed $\bm{x}$, the value of neural network $f_{\bm{\theta}(t)}^{m}$ at $\bm{x}$ converges to the value of the function $f_{t}^{\NTK}$ at $\bm{x}$  with high probability as $m\rightarrow\infty$. Lots of inspired works (see e.g.,{\color{red} citation}\cite{hu2021regularization, suh2022nonparametric}) ignored the subtle difference between the uniformly and pointwisely convergences and claimed that the excess risk of neural network $f_{\bm{\theta}(t)}^{m}(\bm{x})$ can be well approximate the excess risk of the function $f_{t}^{\NTK}(\bm{x})$.
  %The uniform approximation of function is a vital clue for us to investigate the generalization performance of the fully trained overparameterized two-layers ReLU neural networks with the help of NTK regression in a carefree way since generalization performance is related to every draw of $\bm{x}$ from $\mu_{\mathcal{X}}$. 


The proof of Proposition \ref{prop:funct:approx} is deferred to Appendix \ref{app:ntk:approx}. Since $f_{\bm{\theta}(t)}$ and $f_{t}^{\NTK}$ are fully characterized by the equations \eqref{nn:theta:flow}, \eqref{nn:f:flow} and\eqref{ntk:f:flow}, one of the key step we needed in the proof of Proposition \ref{prop:funct:approx} is that the time-varying neural network kernel  $K_{\bm{\theta}(t)}$ uniformly converges  to the time-independent neural tangent kernel $K_{d}$.

% Using Proposition \ref{prop:kernel:approx}, we can further prove the uniform function approximation as follows.

\begin{proposition}\label{prop:kernel:approx}
     Given the training data, if the width $m$ of the two-layers ReLU neural network is sufficiently large, then
    \begin{equation*}
        \sup_{\bm{x},\bm{x}'}\sup_{t\geq 0}| K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K_d(\bm{x},\bm{x}')|=o_{m}(1)
    \end{equation*}
    holds with probability converging to one over initialization as the width $m$ goes to infinity.
\end{proposition}

The proof of Proposition \ref{prop:kernel:approx} is given in Appendix \ref{app:ntk:approx}.  Previous works, such as \cite{jacot2018neural, du2018gradient}, only showed the  time-varying kernel $K_{\bm{\theta}(t)}$ converges pointwisely to the time-independent neural tangent kernel $K_{d}$ as the width $m\rightarrow\infty$.  The significance of this proposition is that it shows that the time-varying kernel $K_{\bm{\theta}(t)}$ converges uniformly to the time-independent neural tangent kernel $K_{d}$ as the width $m\rightarrow\infty$.  Thanks to the uniform convergence result, we are now able to claim that the  excess risk of $f_{\bm{\theta}(t)}^{m}$ is well approximated by the excess risk of $f^{\NTK}_{t}$.


%It is worth emphasizing that Proposition \ref{prop:kernel:approx} states that the uniform approximation of kernel over all $\bm{x},\bm{x}'$ with high probability. Results from the previous works, such as \cite{jacot2018neural, du2018gradient}, could be summarized as the point-wise approximation of the kernel. The problem is that although $K_{\bm{\theta}(t)}(\bm{x},\bm{x}')$ converges to $K_{d}(\bm{x},\bm{x}')$ with high probability, there is no guarantee of uniform convergence with a high probability by simply using the union bound. A more delicate analysis is needed.


\subsection{The generalization performance of overparameterized neural networks over $\mathbb{R}$}\label{subsec:generalization}

% In Section \ref{subsec:ntk:approx}, we have mentioned $f_{\bm{\theta}(t)}$ can be effectively approximated by $f_{t}^{\NTK}$. So we can analyze the generalization performance of $f_{\bm{\theta}(t)}$ via the performance of $f_{t}^{\NTK}$. In this section, we will focus on $f_{t}^{\NTK}$ over $\mathbb{R}$. 
% For $d=1$, $K_{1}(x,x')$ is given by
%     \begin{equation}\label{ntk:L=1:d=1}
%       K_{1}(x,x')= 2\left(1-\psi(x,x')/\pi\right)(x x'+1) +|x-x'| /\pi+1,
%   \end{equation}
% where $\psi(x,x') = \arccos(\frac{xx'+1}{\sqrt{(x^2+1)(x'^2+1)}})\in[0,\frac{\pi}{4}]$.

In Section \ref{subsec:ntk:approx}, we have mentioned $f_{\bm{\theta}(t)}$ can be effectively approximated by $f_{t}^{\NTK}$. So we can analyze the generalization performance of $f_{\bm{\theta}(t)}$ via the performance of $f_{t}^{\NTK}$.  In this section, we focus on data with one-dimensional feature and will show that the fully trained over-parameterized two-layers ReLU neural networks with early stopping is minimax rate optimal, while the neural network trained until overfitting might not even be consistent. 

% Here we give the explicit formula of NTK $K_{1}(x,x')$ for $d=1$ as follows,
%     \begin{equation}\label{ntk:L=1:d=1}
%       K_{1}(x,x')= 2\left(1-\psi(x,x')/\pi\right)(x x'+1) +|x-x'| /\pi+1,
%   \end{equation}
% where $\psi(x,x') = \arccos(\frac{xx'+1}{\sqrt{(x^2+1)(x'^2+1)}})\in[0,\frac{\pi}{4}]$. 

It is well known that the rate of convergence of any estimator can be arbitrarily slow if no restrictions are imposed on the class that the regression function lies in \cite{devroye1996probabilistic}. Hence in our setting, we make the following assumption for the ground true function $f_{\star}$.
%\textcolor{red}{results for regression are needed}
\begin{assumption}\label{assump:f_star}
    $f_{\star}\in \mathcal{H}_{K_1}$ and $\| f_{\star}\|_{\mathcal{H}_{K_{1}}}\leq R$ for some constant $R$, where $K_1$ is the NTK.
\end{assumption}
% explain why this assumption, references, maybe a term for such setup: regression function related to RKHS and estimate based on kernels by spectral algorithm
Assumption \ref{assump:f_star} is very common in the literature for statistical learning theory, see \cite{caponnetto2007optimal, yao2007early, raskutti2014early, blanchard2018optimal, lin2020optimal}. For more applications of RKHS in statistical learning, we refer the readers to \cite{wahba1990spline, saitoh2016theory, scholkopf2018learning}.

\subsubsection{Over-parameterized neural networks are minimax rate optimal with early stopping}

% how to introduce spectral algorithm
% assuming regression function in an RKHS, many kernel based methods/algorithms with. regularization is needed. for example kernel ridge regression(regularized least square), kernel gradient descent?, 

%spectral regularization methods are standard for finding stable solutions for ill-posed inverse problems. to prevent overfitting.

%These have been extensively studied in the literature, for an account see \cite{caponnetto2007optimal, yao2007early, raskutti2014early, blanchard2018optimal, lin2020optimal}, and references therein.
%NTK regression falls into the category of spectral algorithms for kernel.

Regularization is a well-known solution to decrease the generalization error while early stopping was presented as an implicit regularization method in gradient descent \cite{morgan1989generalization, yao2007early}. The generalization of early stopping in kernel methods is widely discussed in previous works \cite{raskutti2014early, lin2020optimal}. In particular, \cite{lin2020optimal} showed that if the eigenvalues satisfy a polynomial decay condition, the kernel methods with early stopping can reach the minimax optimal rate. Thus, with the decay rate of the eigenvalue associated with $K_1$ (Theorem \ref{thm:spectral:d=1:L=1}), the generalization error of $f_t^{\NTK}$ with early stopping can be presented as followed:

\begin{proposition}\label{prop:early:stopping}
    Suppose Assumption \ref{assump:f_star} holds. For the NTK regression, if the training process is stopped at $t_{\star}=\Theta(n^{1/3})$, then
    \begin{equation}
        \excrisk(f_{t_{\star}}^{\NTK})=O(n^{-\frac{2}{3}}\log^{2}\frac{6}{\delta})
    \end{equation}
    holds with probability at least $1-\delta$ over the training data and 
    \begin{equation}
    \inf_{\hat{f}_{n}}\sup_{f_{\star}\in\mathcal{H}_{K_{1}},\| f_{\star}\|_{\mathcal{H}_{K_{1}}}\leq R}\Expc\excrisk(\hat{f}_{n})=\Omega(n^{-\frac{2}{3}}).
    \end{equation}
\end{proposition}



%RKHS regression(regression function in an RKHS) has a long history. inverse problem. more complicated source condition.

%hardness is determined by the lower bound of the eigenvalue decay rate. upper bound of the eigenvalue decay the bound for a specific algorithm.


% some words or not

% many researchers are aware that neural networks need some regularization to generalize well

% early stopping in machine learning other than neural networks

% works that are related to NN early stopping? \cite{ji2021earlystopped, li2020gradient, li2021implicit}

%gradient flow is one of the spectral algorithms. and the optimal stopping time relies on the eigenvalue decay rate. 

% however, \cite{raskutti2014early} provides a data-depesndent optimal stopping time, in this case one does not need to know the decay rate in advance. a little bug

%According to Proposition \ref{prop:minimax:lower:bound} and Proposition \ref{prop:early:stopping:rate}, NTK polynomial decay. so combining these

%Theorem \ref{thm:spectral:d=1:L=1} gives guidance on choosing the optimal stopping time. 

% In this section, Theorem \ref{thm:nn:early:stopping:d=1} rigorously shows the fully trained over-parameterized two-layers ReLU neural networks with early stopping is minimax rate optimal, which is the first result to the best of our knowledge.

With Theorem \ref{thm:risk:approx} controlling the gap between the generalization error of $f_{t}^{\NTK}$ and the one of $f_{\bm{\theta}(t)}$, we can bound the generalization error of neural networks with early stopping.

\begin{theorem}\label{thm:nn:early:stopping:d=1}
    If the width $m$ of the two-layers ReLU neural network is sufficiently large and the training process is stopped at $t_{\star} =\Theta(n^{1/3})$, then
    \begin{equation*}
        \excrisk(f_{\bm{\theta}(t_{\star})})=O(n^{-\frac{2}{3}\log^{2}\frac{6}{\delta}})
    \end{equation*}
    holds with probability converging to one over initialization and with probability at least $1-\delta$ over the training data.
\end{theorem}

%\begin{proof}
%    Theorem \ref{thm:risk:approx} and Proposition \ref{prop:early:stopping:rate}.
%\end{proof}

Theorem \ref{thm:nn:early:stopping:d=1} rigorously shows the fully trained over-parameterized two-layers ReLU neural networks with early stopping is minimax rate optimal. However, in the absence of early stopping, the following result shows the poor performance of over-parameterized neural networks.

% Lin et al. \cite{lin2020optimal} have considered the regression problem (Equation \eqref{equation:true_model}). They investigated the generalization performance of the solution obtained by the gradient descent method with $0\in \mathcal{H}_{\Phi}$ as the initialization point(function). They showed that a properly chosen early stopping strategy leads to a minimax optimal solution if we know the decay rate of eigenvalues of the kernel. Proposition \ref{prop:early:stopping} is a direct consequence from \cite{lin2020optimal} by applying Lemma \ref{thm:spectral:d=1:L=1}.

% add

% try to find the first work that gives the upper bound of RKHS regression. lin2020optimal is too general

% Combining Proposition \ref{prop:early:stopping} and Theorem \ref{thm:risk:approx}, Corollary \ref{thm:nn:early:stopping} follows, indicating the overparameterized two-layer neural network with early stopping is minimax rate optimal.

\subsubsection{Over-fitted Neural Networks generalize poorly}

We are interested in the behavior of $f^{\NTK}_{t}$ when $t$ is sufficiently large, which represents over-fitted neural networks. Given the specific kernel $K$, we can consider Kernel Ridgeless Regression, which is presented as

\begin{equation}\label{eq:ridgeless}
    f(x) = K(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}.
\end{equation}

 In the absence of explicit regularization, Kernel Ridgeless Regression with nonlinear kernels has the potential to fit the data points perfectly. The kernel can be chosen like RBF kernel or polynomial kernel. Compared with Equation \eqref{ntk:solution} and \eqref{eq:ridgeless}, as $t\to\infty$, Equation \eqref{ntk:solution} becomes Kernel Ridgeless Regression with NTK. Thus, we will discuss the behavior of $f^{\NTK}_{\infty}(x) = K_1(x,\bm{X})K_1^{-1}(\bm{X},\bm{X})\bm{y}$, which represents over-fitted neural networks that can interpolate the data points.

To be more concrete, we consider the equally-distanced one-dimensional data $\{\bm{X},\bm{y}\}=\{(x_{i},y_{i}) \mid x_{i}=\frac{i-1}{n-1}, i \in [n]\}$ as an example. We will focus on the performance of $f^{\NTK}_{\infty}(x)$ on such data. Before analyzing the generalization performance, a special property of $f^{\NTK}_{\infty}(x)$ should be highlighted:

\begin{proposition}[Bounded second order derivative of over-fitted NTK regression]\label{prop:bound_second_derivative}
Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. With the probability at least $1-\frac{2}{n}$, we have
\begin{align}
 \sup_{x\in (x_i,x_{i+1})}|K_1''(x,\bm{X})K_1^{-1}(\bm{X},\bm{X})\bm{y}|\leq C\sqrt{\log(n)} 
\end{align}
 for $\forall i\in[n]$ and for some constant $C$.
\end{proposition}
\begin{remark}
If we assume all the labels $\bm{y}$ are bounded(e.g., classification problems), i.e., $|y_i|\leq C$, $ j\in[n]$, the upper bound of Proposition \ref{prop:bound_second_derivative} will be a constant $C$ instead of $C\sqrt{\log(n)}$. Proposition \ref{prop:bound_second_derivative} is infrequent in many kernels such as Gaussian kernel or Polynomial kernel. 
\end{remark}

Let
\begin{align}
    f_{\LI}(x)=y_{i}+\frac{y_{i+1}-y_{i}}{x_{i+1}-x_{i}}(x-x_{i}), \mbox{ when } x\in [x_{i},x_{i+1}]
\end{align}
be the linear interpolation of these $n$ points. By Taylor expansion, Proposition \ref{prop:bound_second_derivative} can guarantee that the linear interpolation can approximate the model as $n$ is increasing. Since the generalization error of the linear interpolation has a constant lower bound on the noisy data. Thus, we have the following theorem:

\begin{theorem}[Overfitted network generalizes poorly]\label{thm:bad_gen}
    Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. With the probability at least $1-\frac{2}{n}$, $f_{\infty}^{\NTK}(x)$ can be approximated by the linear interpolation, i.e.,
\begin{align}
 \sup_{x\in [0,1]}|f^{\NTK}_{\infty}(x)-f_{\LI}(x)|\leq C\sqrt{\log(n)} /(n-1)^{2}
\end{align}
for some constant $C$. Moreover, the generalization error of $f_{\infty}^{\NTK}(x)$ is bounded away from zero, i.e.,
    \begin{equation}
       \excrisk(f_{\infty}^{\NTK}) \geq  C
    \end{equation}
 for some constant $C$.
\end{theorem}

\begin{remark}
 To the best of our knowledge, it is the first time to show how wide neural networks interpolate on the data. Combined with Proposition \ref{prop:funct:approx} and Theorem \ref{thm:bad_gen}, our theory shows that for over-fitted neural networks, adding more parameters does not increase the model complexity but makes the models more concise. The experiment results are shown in Figure \ref{fig:LI} (a). That is the reason why over-fitted neural networks can not affect too much by overparameterization.
\end{remark}

\begin{remark}
The second result of Theorem \ref{thm:bad_gen} is to give an example showing that the overfitted neural network can have bad generalization, which contradicts the observation  {\bf (S)}. Since the lower bound $C$ in Theorem \ref{thm:bad_gen} is related to the scale of the noise, we believe the overfitted neural network can not generalize well in most cases unless the noise is small enough. Figure \ref{fig: d_larger_than_1} (b) gives more examples showing that, even for $d>1$, the generalization error of overfitted networks is bounded away from zero even if the sample size is increasing.
\end{remark}

 Different from RBF kernel (or high order polynomial kernel) ridgeless regression,  Figure \ref{fig:LI} (a) and (b) present that the interpolation ways of the overfitted NTK model $f^{\NTK}_{\infty}(x)$ and wide neural network are nearly linear. Theorem \ref{thm:bad_gen} gives the upper bound of the gap between the overfitted NTK model and the linear interpolation is $O(\frac{1}{n^2})$ while Figure \ref{fig:LI} (c) shows that the gap actually is exactly $O(\frac{1}{n^2})$. These experimental results are in line with the conclusions of Proposition \ref{prop:funct:approx} and Theorem \ref{thm:bad_gen}.

\begin{figure}[htbp]
    \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{NN_with_diff_m.png}
      \centerline{(a)}
  \end{minipage}%
  \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{LI_NTK_RBF.png}
      \centerline{(b)}
  \end{minipage}%
  \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{gap_between_NTK_LI.png}
      \centerline{(c)}
  \end{minipage}
  \caption{(a): The interpolation ways of one-hidden-layer neural networks with different widths; (b): The interpolation ways of linear interpolation, $f^{NTK}_{\infty}(x)$ and RBF kernel regression with $\gamma=1$; (c): The gap between $f^{NTK}_{\infty}(x)$ and linear interpolation. The input of the training data is the equally-distanced one-dimensional data $\{x_{i}=\frac{i-1}{n-1}, i \in [n]\}$. The label of the training data is randomly selected from $\{1,-1\}$, which does not contribute to the experiment result. The sample size $n=100,200,...,1000$}\label{fig:LI}
\end{figure}





























\begin{comment}
\subsection{Speculation on $\mathbb{R}^{d}$}

\begin{figure}[htbp]
    \begin{minipage}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\textwidth]{min_eigenvalue_for_diff_d}
        \centerline{(a) Minimum eigenvalue of NTK}
    \end{minipage}%
    \begin{minipage}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\textwidth]{test_error_of_NTK.png}
        \centerline{(b) Generalization error for Overfitted Neural Networks}
    \end{minipage}
    \caption{(a) Minimum eigenvalue of NTK on $\mathbb{R}^{d}$: The input is the equally-distanced data $\{\bm{x}_i\}_{i=1}^n$, defined as $\{(\frac{i_1-1}{n_d-1},...,\frac{i_d-1}{n_d-1})\}$, $i_1,...,i_d\in[n_d]$, where $n_d=n^{\frac{1}{d}}$. We calculate the minimum eigenvalue of NTK with different minimum distances $\frac{1}{n_d-1}$; (b) Generalization error for Overfitted NTK $f^{\NTK}_{\infty}$ over $\mathbb{R}^{d}$: The input $x \sim \unif(0,1)^d$ where $d=2,3,4$. $f_{\star}(x) = \sin(\frac{\sum_{j=1}^{d}x_j}{\sqrt{d}})$ and $y=f_{\star}(x)+0.1\varepsilon$, where $\varepsilon \sim N(0,1)$. The sample size of training data $n=100,300,500,...,1900$ and the number of testing data is $1000$ for all experiments.}
    \label{fig: d_larger_than_1}
  \end{figure}

\subsubsection*{Spectral properties of NTK} The experiment of the minimum eigenvalue is presented in Figure \ref{fig: d_larger_than_1} (a), showing that for fixed $d$, the minimum eigenvalue $\lambda_{\min}$ of $K_d(\bm{X},\bm{X})$ tends to be $\Theta(d_{\min})$, i.e., $c d_{\min}\leq \lambda_{\min} \leq C d_{\min}$ for some constants $c$ and $C$. 

\cite{bietti2019inductive} has shown that on $\mathbb{S}^{d-1}$, the eigenvalues associated with the bias-free NTK $\lambda_k \asymp k^{-\frac{d}{d-1}}$ (considering multiple roots). There are some zero eigenvalues for the bias-free NTK and adding a bias may prevent such zero eigenvalues. Thus, we believe that on $\mathbb{R}^{d}$, the eigenvalues of the NTK with biases $\lambda_k \asymp k^{-\frac{d+1}{d}}$. This conjecture is the key to the generalization ability of neural networks with early stopping.



\subsubsection*{Over-parameterized neural networks are minimax rate optimal with early stopping} We can make the following assumptions:
\begin{assumption}\label{assumption:EDR_for_R_d}
    Let $\lambda_j,j=0,1,2\dots$ be the eigenvalues associated with the NTK $K_d$ defined on $[0,1]^{d}$ and satisfies
\begin{equation}
    \lambda_{j} \asymp j^{-\frac{d+1}{d}}.
\end{equation}
\end{assumption}
\begin{assumption}\label{assumption:f_star_in_H_K_d}
    $f_{\star}\in \mathcal{H}_{K_d}$ where $K_d$ is the NTK.
\end{assumption}
Then with these two assumptions, we have the following results:
\begin{proposition}\label{prop:early:stopping:d} 
Suppose Assumption \ref{assumption:EDR_for_R_d} and \ref{assumption:f_star_in_H_K_d} hold. For the NTK regression, if we stop the training process at  $t_{\star}=\Theta(n^{-(d)/(2d+1)})$, then
\begin{equation}
     \excrisk(f_{t_{\star}}^{\NTK})=O( n^{-(d+1)/(2d+1)}\log^{2}\frac{6}{\delta}),
\end{equation}
with probability at least $1-\delta$ and
\begin{equation}
    \inf_{\hat{f}_{n}}\sup_{f_{\star}\in\mathcal{H}_{K},\lVert f_{\star}\rVert\leq R}\Expc\excrisk(\hat{f}_{n}) =\Omega( n^{-(d+1)/(2d+1)}).
\end{equation}
\end{proposition}
Thus, combined with Theorem \ref{thm:risk:approx}, we show the generalization performance of neural networks with early stopping.


\subsubsection*{Over-fitted neural networks generalize poorly}  The experiment of the generalization error is presented in Figure \ref{fig: d_larger_than_1} (b), showing that for fixed $d$, the generalization error of $f^{\NTK}_{\infty}$ is bounded away from zero even when $n$ is increasing.

In summary, for fixed $d$, the conjectures on the $\mathbb{R}^{d}$ are summarized as followed:

i) Let $\bm{X} = \{\bm{x}_i,...,\bm{x}_n\}\in [0,1]^{d}$ and $d_{\min} = \min_{i\neq j}\|\bm{x}_i-\bm{x}_j\|$. The minimum eigenvalue, $\lambda_{\min}$ of $K_d(\bm{X},\bm{X})$ satisfies 

\begin{equation}
    \lambda_{\min} \asymp d_{\min}
\end{equation}
for some constants $c$, $C$.

ii) Let $\lambda_j,j=0,1,2\dots$ be the eigenvalues associated with the NTK $K_d$ defined on $[0,1]^{d}$ and satisfies
\begin{equation}
    \lambda_{j} \asymp j^{-\frac{d+1}{d}}.
\end{equation}

iii) Assume ii) holds and $f_{\star} \in \mathcal{H}_{K_d}$, then if the width $m$ of the two-layers ReLU neural network is sufficiently large and the training process is stopped at $t_{\star}=\Theta(n^{-(d)/(2d+1)})$, then
    \begin{equation*}
        \excrisk(f_{\bm{\theta}(t_{\star})})=O( n^{-(d+1)/(2d+1)}\log^{2}\frac{6}{\delta}),
    \end{equation*}
    with probability converging to one over initialization and high probability over the training data.

iv) The generalization error of the over-fitted NTK model with zero initialization is bounded away from zero, i.e.,
    \begin{equation}
       \excrisk(f_{\infty}^{\NTK}) \geq  C
    \end{equation}
 for some constant $C$.
\end{comment}




















==> main_result.tex <==
To simplify the mathematical argument, we consider the gradient flow of neural networks. The gradient flow in $\bm{\Theta}$ induced by the loss function is given by
\begin{equation}
\begin{aligned}
      \dot{\bm{\theta}}(t) &=\frac{\dx}{\dx t}\bm{\theta}(t)=-\nabla_{\bm{\theta}}\emprisk(f_{\bm{\theta}})= - \frac{1}{n}\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})\tran (f_{\bm{\theta}(t)}(\bm{X})-\bm{y})
\end{aligned}
\end{equation}
where $\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})$ is an $n\times ((d+2)m+1)$ matrix.
This flow induced an associated flow in  $\mathcal{F}^{m}$:    
\begin{equation}\label{nn:f:flow}
\begin{aligned} 
\dot{f}_{\bm{\theta}(t)}(\bm{x}) &=\frac{\dx }{\dx t}f_{\bm{\theta}(t)}(\bm{x})=\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{x})\dot{\bm{\theta}}(t)= -\frac{1}{n} K_{\bm{\theta}(t)}(\bm{x},\bm{X}) (f_{\bm{\theta}(t)}(\bm{X})-\bm{y}),
\end{aligned}
\end{equation}
where $K_{\bm{\theta}(t)}(\bm{x},\bm{X}) =\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{x}) \nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})\tran$. We often refer to $K_{\bm{\theta}(t)}$ as the neural network kernel which is a time-varying kernel.  

With the gradient flow of Equation \eqref{nn:f:flow}, the neural network function can be determined by the initialization $f_{\bm{\theta}(0)}(\bm{x})$. However, $f_{\bm{\theta}(0)}(\bm{x})$ is random because of the initialization of the parameters and the randomness of $f_{\bm{\theta}(0)}(\bm{x})$ is irrelevant to the data set. To eliminate effect of the randomness, we can assume $f_{\bm{\theta}(0)}(\bm{x})$ is small, i.e., $f_{\bm{\theta}(0)}(\bm{x})\approx 0$. This can be ensured by replicating a network with the same values on the first layer and opposite signs on the top layer at initialization and the bias term on the top layer is set as zero. More specifically, for $2m$, we can initialize the parameters $a_{r}(0),\bm{w}_{r,j}(0),b_{r}(0), \sim \mathcal{N}(0,1)$ for $r\in [m]$, $j\in [d]$, $a_{r+m}(0)=a_{r}(0)$, $\bm{w}_{r+m,j}(0)=\bm{w}_{r,j}(0)$, $b_{r+m}(0)=b_{r}(0)$ and $b =0$. With this initialization, $f_{\bm{\theta}(0)}(\bm{x})=0$.

\vspace{3mm}

Since Equation \eqref{nn:f:flow} is highly non-linear and hard to find an explicit solution, various approximated solutions \cite{mei2019mean, karakida2019universal, sirignano2022mean, eldan2021non} were proposed to characterize the asymptotic behavior of these equations. In the seminal paper, Jacot et al\cite{jacot2018neural} observed that for any $t$,
\begin{align}
    K_{\bm{\theta}(t)}(\bm{x},\bm{x}')\xrightarrow{m\rightarrow \infty} K_d(\bm{x},\bm{x}')
\end{align}
where $K_d(\bm{x},\bm{x}')$ is a time-independent kernel on $\mathbb{R}^d\times \mathbb{R}^d$. This kernel, now often referred to as the neural tangent kernel (NTK), leads us to consider the following gradient flow of NTK regression
\begin{equation}\label{ntk:f:flow}
    \begin{aligned}
    \dot{f}^{\NTK}_{t}(\bm{x})=\frac{\dx}{\dx t}f^{\NTK}_{t}(\bm{x})=-\frac{1}{n}K_d(\bm{x},\bm{X})(f^{\NTK}_{t}(\bm{X})-\bm{y})
    \end{aligned}
\end{equation}
in the space $\mathcal{F}$, the RKHS associated to the kernel $K$. $K_d(\bm{x},\bm{X}) = (K_d(\bm{x},\bm{x}_1),\dots,K_d(\bm{x},\bm{x}_n))\in \mathbb{R}^{1\times n}$. Similar to the neural network function, we assume $f^{\NTK}_{0}(\bm{x})=0$. Though it is hard to analyze the solution $f_{\bm{\theta}(t)}$ of the equation \eqref{nn:f:flow} directly, we may focus on the solution $f^{\NTK}_{t}$ of the equation \eqref{ntk:f:flow} first if $m$ is sufficiently large. This simplifies the problem substantially, as we can solve the equation \eqref{ntk:f:flow} explicitly: 
\begin{equation}\label{ntk:solution}
    f_t^{\NTK}(\bm{x})=K_d(\bm{x},\bm{X})K_d(\bm{X},\bm{X})^{-1}(\bm{I}-e^{-\frac{1}{n}K_d(\bm{X},\bm{X})t})\bm{y}
\end{equation}
The uniform approximation between $f^{\NTK}_{t}(\bm{x})$ and $f_{\bm{\theta}(t)}$ will be presented in the next subsection.

\subsection{Uniform NTK approximation for over-parameterized neural networks}\label{subsec:ntk:approx}

% One may naturally expect that the solution $f_{\bm{\theta}(t)}$ of the equation \eqref{nn:f:flow} and the solution $f^{\NTK}_{t}$ of the equation \eqref{ntk:f:flow} should behave in a similar way for sufficiently large $m$.  
% Furthermore, when $m$ is sufficiently large, 
% some researchers often referred to the flow $f_{\bm{\theta}(t)}$ as the lazy trained neural network, for 
% the movement of $\bm{\theta}(t)$ is ignorable in this scenario (e.g., \cite{lee2019wide},\cite{du2018gradient},\cite{jacot2018neural}).
% These statements have been justified in a sequence of works from various groups of researchers (see e.g., \cite{jacot2018neural},\cite{arora2019exact},\cite{lee2019wide}). 

% #comparisons with other similar work

% We are aware that \cite{hu2021regularization}, \cite{suh2022nonparametric} have shown that the generalization error of the neural network trained for too long is bounded away from zero. However, it is worth noting that both of their results need NTK regression as an intermediate term. Then it is necessary to prove that the generalization error of the neural network could be approximated by that of NTK regression.

% why uniform NTK approximation is important

Since the seminal work \cite{jacot2018neural} brought up the concept of the NTK, many works have been trying to understand the generalization performance of neural networks based on the NTK \cite{vyas2022limitations, arora2019exact, arora2019fine, hu2021regularization, suh2022nonparametric, montanari2022interpolation}. In this subsection, we show that the generalization performance of the over-parameterized two-layers ReLU neural networks $f_{\bm{\theta}(t)}$ could be studied via NTK regression $f_{t}^{\NTK}$ and the precise argument is established in Theorem \ref{thm:risk:approx}, paving the way for the discussion about generalization performance of neural networks in Section \ref{subsec:generalization}. 

% With Theorem \ref{thm:risk:approx}, using NTK regression as a substitute to investigate the generalization performance of the over-parameterized two-layers ReLU neural network is rigorously valid. 

% In the following Section \ref{subsec:generalization}, the generalization performance of the fully trained overparameterized two-layers ReLU neural networks could be understood with the help of NTK regression in a carefree way.

% To the best of our knowledge, we give the first concrete result on that the generalization error of the fully trained two-layers ReLU neural networks could be represented by NTK regression, which is our Theorem \ref{thm:risk:approx}.

\begin{theorem}\label{thm:risk:approx}
    Given the training data, for all $t\geq 0$, if the width $m$ of the two-layers ReLU neural network is sufficiently large, then
    \begin{equation*}
        |\excrisk(f_{\bm{\theta}(t)})-\excrisk(f_{t}^{\NTK})|=o_{m}(1)
    \end{equation*}
    holds with probability converging to one over initialization as the width $m$ goes to infinity. 
\end{theorem}

\begin{proof}
    Plugging in $f_{t}^{\NTK}$ in the excess risk of the two-layers ReLU neural network $\excrisk(f_{\bm{\theta}(t)})$ according to \eqref{eq:excrisk} shows $\excrisk(f_{\bm{\theta}(t)})-\excrisk(f_{t}^{\NTK})$ could be controlled by upper bounding   $\int_{\mathcal{X}}(f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x}))^{2}\dx\mu_{\mathcal{X}}(\bm{x})$ and $\int_{\mathcal{X}}(f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x}))(f_{t}^{\NTK}(\bm{x})-f_{\star}(\bm{x}))\dx \mu_{\mathcal{X}}(\bm{x})$. The term $\sup_{\bm{x}}|f_{t}^{\NTK}(\bm{x})-f_{\star}(\bm{x})|$ could be bounded by arguing that $f_{t}^{\NTK}$ and $f_{\star}$ are both continuous over the compact set $\mathcal{X}$. Thus
    \begin{equation*}
        |\excrisk(f_{\bm{\theta}(t)})-\excrisk(f_{t}^{\NTK})|=O(\sup_{\bm{x}}|f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})|),
    \end{equation*}
    indicating the uniform approximation of $f_{t}^{\NTK}$ to $f_{\bm{\theta}(t)}$, i.e., $\sup_{\bm{x}}|f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})|$ lies at the heart of the proof of Theorem \ref{thm:risk:approx}, which is provided in Proposition \ref{prop:funct:approx} below.
\end{proof}

% to prove this theorem, emphasize the importance of uniform convergence.

% A closer look at \eqref{eq:excrisk} suggests , since the generalization is related to all possible $\bm{x}$ drawn from $\mu_{X}$.

\begin{proposition}\label{prop:funct:approx}
    Given the training data, if the width $m$ of the two-layers ReLU neural network is sufficiently large, then for all $t\geq 0$, 
    \begin{equation*}
        \sup_{\bm{x}}| f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})|=o_{m}(1)
    \end{equation*}
    holds with probability converging to one over initialization as the width $m$ goes to infinity.
\end{proposition}

% Check
% \begin{itemize}
%     \item $\alpha<1/2$
%     \item $1-\gamma<\beta/2$
%     \item $\gamma>\max\{1-\alpha,\delta\}$
%     \item $\beta>\alpha$
% \end{itemize}

\begin{remark}
    Proposition \ref{prop:funct:approx} shows the difference between $f_{\bm{\theta}(t)}(\bm{x})$ and $f_{t}^{\NTK}(\bm{x})$ over all $\bm{x}$ can be controlled uniformly with high probability by the width $m$, compared to similar results by \cite{lee2019wide, arora2019exact}. The uniform approximation of function is a vital clue for us to investigate the generalization performance of the fully trained overparameterized two-layers ReLU neural networks with the help of NTK regression in a carefree way since generalization performance is related to every draw of $\bm{x}$ from $\mu_{\mathcal{X}}$. 
\end{remark}

The proof of Proposition \ref{prop:funct:approx} is deferred to Appendix \ref{app:ntk:approx}. Since \eqref{nn:f:flow} and \eqref{ntk:f:flow} imply the evolution of $f_{\bm{\theta}(t)}$ and $f_{t}^{\NTK}$ is fully determined by the kernel $K_{\bm{\theta}(t)}$ and $K_{d}$ respectively, it suffices to give the uniform approximation of $K_{\bm{\theta}}$ to $K_{d}$ in Proposition \ref{prop:kernel:approx} below in order to prove Proposition \ref{prop:funct:approx}.

% Using Proposition \ref{prop:kernel:approx}, we can further prove the uniform function approximation as follows.

\begin{proposition}\label{prop:kernel:approx}
     Given the training data, if the width $m$ of the two-layers ReLU neural network is sufficiently large, then
    \begin{equation*}
        \sup_{\bm{x},\bm{x}'}\sup_{t\geq 0}| K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K_d(\bm{x},\bm{x}')|=o_{m}(1)
    \end{equation*}
    holds with probability converging to one over initialization as the width $m$ goes to infinity.
\end{proposition}
The proof of Proposition \ref{prop:kernel:approx} is given in Appendix \ref{app:ntk:approx}. 

\begin{remark}
    It is worth emphasizing that Proposition \ref{prop:kernel:approx} implies the uniform approximation of kernel over all $\bm{x},\bm{x}'$ with high probability. Results from the previous works, such as \cite{jacot2018neural, du2018gradient}, could be summarized as the point-wise approximation of the kernel. The problem is that although $K_{\bm{\theta}(t)}(\bm{x},\bm{x}')$ converges to $K_{d}(\bm{x},\bm{x}')$ with high probability, there is no guarantee of uniform convergence with a high probability by simply using the union bound. A more delicate analysis is needed.
\end{remark}

\subsection{The generalization performance of overparameterized neural networks over $\mathbb{R}$}\label{subsec:generalization}

% In Section \ref{subsec:ntk:approx}, we have mentioned $f_{\bm{\theta}(t)}$ can be effectively approximated by $f_{t}^{\NTK}$. So we can analyze the generalization performance of $f_{\bm{\theta}(t)}$ via the performance of $f_{t}^{\NTK}$. In this section, we will focus on $f_{t}^{\NTK}$ over $\mathbb{R}$. 
% For $d=1$, $K_{1}(x,x')$ is given by
%     \begin{equation}\label{ntk:L=1:d=1}
%       K_{1}(x,x')= 2\left(1-\psi(x,x')/\pi\right)(x x'+1) +|x-x'| /\pi+1,
%   \end{equation}
% where $\psi(x,x') = \arccos(\frac{xx'+1}{\sqrt{(x^2+1)(x'^2+1)}})\in[0,\frac{\pi}{4}]$.

In Section \ref{subsec:ntk:approx}, we have mentioned $f_{\bm{\theta}(t)}$ can be effectively approximated by $f_{t}^{\NTK}$. So we can analyze the generalization performance of $f_{\bm{\theta}(t)}$ via the performance of $f_{t}^{\NTK}$.  In this section, we focus on data with one-dimensional feature and will show that the fully trained over-parameterized two-layers ReLU neural networks with early stopping is minimax rate optimal, while the neural network trained until overfitting might not even be consistent. 

% Here we give the explicit formula of NTK $K_{1}(x,x')$ for $d=1$ as follows,
%     \begin{equation}\label{ntk:L=1:d=1}
%       K_{1}(x,x')= 2\left(1-\psi(x,x')/\pi\right)(x x'+1) +|x-x'| /\pi+1,
%   \end{equation}
% where $\psi(x,x') = \arccos(\frac{xx'+1}{\sqrt{(x^2+1)(x'^2+1)}})\in[0,\frac{\pi}{4}]$. 

It is well known that the rate of convergence of any estimator can be arbitrarily slow if no restrictions are imposed on the class that the regression function lies in \cite{devroye1996probabilistic}. Hence in our setting, we make the following assumption for the ground true function $f_{\star}$.
%\textcolor{red}{results for regression are needed}
\begin{assumption}\label{assump:f_star}
    $f_{\star}\in \mathcal{H}_{K_1}$ and $\| f_{\star}\|_{\mathcal{H}_{K_{1}}}\leq R$ for some constant $R$, where $K_1$ is the NTK.
\end{assumption}
% explain why this assumption, references, maybe a term for such setup: regression function related to RKHS and estimate based on kernels by spectral algorithm
Assumption \ref{assump:f_star} is very common in the literature for statistical learning theory, see \cite{caponnetto2007optimal, yao2007early, raskutti2014early, blanchard2018optimal, lin2020optimal}. For more applications of RKHS in statistical learning, we refer the readers to \cite{wahba1990spline, saitoh2016theory, scholkopf2018learning}.

\subsubsection{Over-parameterized neural networks are minimax rate optimal with early stopping}

% how to introduce spectral algorithm
% assuming regression function in an RKHS, many kernel based methods/algorithms with. regularization is needed. for example kernel ridge regression(regularized least square), kernel gradient descent?, 

%spectral regularization methods are standard for finding stable solutions for ill-posed inverse problems. to prevent overfitting.

%These have been extensively studied in the literature, for an account see \cite{caponnetto2007optimal, yao2007early, raskutti2014early, blanchard2018optimal, lin2020optimal}, and references therein.
%NTK regression falls into the category of spectral algorithms for kernel.

Regularization is a well-known solution to decrease the generalization error while early stopping was presented as an implicit regularization method in gradient descent \cite{morgan1989generalization, yao2007early}. The generalization of early stopping in kernel methods is widely discussed in previous works \cite{raskutti2014early, lin2020optimal}. In particular, \cite{lin2020optimal} showed that if the eigenvalues satisfy a polynomial decay condition, the kernel methods with early stopping can reach the minimax optimal rate. Thus, with the decay rate of the eigenvalue associated with $K_1$ (Theorem \ref{thm:spectral:d=1:L=1}), the generalization error of $f_t^{\NTK}$ with early stopping can be presented as followed:

\begin{proposition}\label{prop:early:stopping}
    Suppose Assumption \ref{assump:f_star} holds. For the NTK regression, if the training process is stopped at $t_{\star}=\Theta(n^{1/3})$, then
    \begin{equation}
        \excrisk(f_{t_{\star}}^{\NTK})=O(n^{-\frac{2}{3}}\log^{2}\frac{6}{\delta})
    \end{equation}
    holds with probability at least $1-\delta$ over the training data and 
    \begin{equation}
    \inf_{\hat{f}_{n}}\sup_{f_{\star}\in\mathcal{H}_{K_{1}},\| f_{\star}\|_{\mathcal{H}_{K_{1}}}\leq R}\Expc\excrisk(\hat{f}_{n})=\Omega(n^{-\frac{2}{3}}).
    \end{equation}
\end{proposition}



%RKHS regression(regression function in an RKHS) has a long history. inverse problem. more complicated source condition.

%hardness is determined by the lower bound of the eigenvalue decay rate. upper bound of the eigenvalue decay the bound for a specific algorithm.


% some words or not

% many researchers are aware that neural networks need some regularization to generalize well

% early stopping in machine learning other than neural networks

% works that are related to NN early stopping? \cite{ji2021earlystopped, li2020gradient, li2021implicit}

%gradient flow is one of the spectral algorithms. and the optimal stopping time relies on the eigenvalue decay rate. 

% however, \cite{raskutti2014early} provides a data-depesndent optimal stopping time, in this case one does not need to know the decay rate in advance. a little bug

%According to Proposition \ref{prop:minimax:lower:bound} and Proposition \ref{prop:early:stopping:rate}, NTK polynomial decay. so combining these

%Theorem \ref{thm:spectral:d=1:L=1} gives guidance on choosing the optimal stopping time. 

% In this section, Theorem \ref{thm:nn:early:stopping:d=1} rigorously shows the fully trained over-parameterized two-layers ReLU neural networks with early stopping is minimax rate optimal, which is the first result to the best of our knowledge.

With Theorem \ref{thm:risk:approx} controlling the gap between the generalization error of $f_{t}^{\NTK}$ and the one of $f_{\bm{\theta}(t)}$, we can bound the generalization error of neural networks with early stopping.

\begin{theorem}\label{thm:nn:early:stopping:d=1}
    If the width $m$ of the two-layers ReLU neural network is sufficiently large and the training process is stopped at $t_{\star} =\Theta(n^{1/3})$, then
    \begin{equation*}
        \excrisk(f_{\bm{\theta}(t_{\star})})=O(n^{-\frac{2}{3}\log^{2}\frac{6}{\delta}})
    \end{equation*}
    holds with probability converging to one over initialization and with probability at least $1-\delta$ over the training data.
\end{theorem}

%\begin{proof}
%    Theorem \ref{thm:risk:approx} and Proposition \ref{prop:early:stopping:rate}.
%\end{proof}

Theorem \ref{thm:nn:early:stopping:d=1} rigorously shows the fully trained over-parameterized two-layers ReLU neural networks with early stopping is minimax rate optimal. However, in the absence of early stopping, the following result shows the poor performance of over-parameterized neural networks.

% Lin et al. \cite{lin2020optimal} have considered the regression problem (Equation \eqref{equation:true_model}). They investigated the generalization performance of the solution obtained by the gradient descent method with $0\in \mathcal{H}_{\Phi}$ as the initialization point(function). They showed that a properly chosen early stopping strategy leads to a minimax optimal solution if we know the decay rate of eigenvalues of the kernel. Proposition \ref{prop:early:stopping} is a direct consequence from \cite{lin2020optimal} by applying Lemma \ref{thm:spectral:d=1:L=1}.

% add

% try to find the first work that gives the upper bound of RKHS regression. lin2020optimal is too general

% Combining Proposition \ref{prop:early:stopping} and Theorem \ref{thm:risk:approx}, Corollary \ref{thm:nn:early:stopping} follows, indicating the overparameterized two-layer neural network with early stopping is minimax rate optimal.

\subsubsection{Over-fitted Neural Networks generalize poorly}

We are interested in the behavior of $f^{\NTK}_{t}$ when $t$ is sufficiently large, which represents over-fitted neural networks. Given the specific kernel $K$, we can consider Kernel Ridgeless Regression, which is presented as

\begin{equation}\label{eq:ridgeless}
    f(x) = K(x,\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}.
\end{equation}

 In the absence of explicit regularization, Kernel Ridgeless Regression with nonlinear kernels has the potential to fit the data points perfectly. The kernel can be chosen like RBF kernel or polynomial kernel. Compared with Equation \eqref{ntk:solution} and \eqref{eq:ridgeless}, as $t\to\infty$, Equation \eqref{ntk:solution} becomes Kernel Ridgeless Regression with NTK. Thus, we will discuss the behavior of $f^{\NTK}_{\infty}(x) = K_1(x,\bm{X})K_1^{-1}(\bm{X},\bm{X})\bm{y}$, which represents over-fitted neural networks that can interpolate the data points.

To be more concrete, we consider the equally-distanced one-dimensional data $\{\bm{X},\bm{y}\}=\{(x_{i},y_{i}) \mid x_{i}=\frac{i-1}{n-1}, i \in [n]\}$ as an example. We will focus on the performance of $f^{\NTK}_{\infty}(x)$ on such data. Before analyzing the generalization performance, a special property of $f^{\NTK}_{\infty}(x)$ should be highlighted:

\begin{proposition}[Bounded second order derivative of over-fitted NTK regression]\label{prop:bound_second_derivative}
Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. With the probability at least $1-\frac{2}{n}$, we have
\begin{align}
 \sup_{x\in (x_i,x_{i+1})}|K_1''(x,\bm{X})K_1^{-1}(\bm{X},\bm{X})\bm{y}|\leq C\sqrt{\log(n)} 
\end{align}
 for $\forall i\in[n]$ and for some constant $C$.
\end{proposition}
\begin{remark}
If we assume all the labels $\bm{y}$ are bounded(e.g., classification problems), i.e., $|y_i|\leq C$, $ j\in[n]$, the upper bound of Proposition \ref{prop:bound_second_derivative} will be a constant $C$ instead of $C\sqrt{\log(n)}$. Proposition \ref{prop:bound_second_derivative} is infrequent in many kernels such as Gaussian kernel or Polynomial kernel. 
\end{remark}

Let
\begin{align}
    f_{\LI}(x)=y_{i}+\frac{y_{i+1}-y_{i}}{x_{i+1}-x_{i}}(x-x_{i}), \mbox{ when } x\in [x_{i},x_{i+1}]
\end{align}
be the linear interpolation of these $n$ points. By Taylor expansion, Proposition \ref{prop:bound_second_derivative} can guarantee that the linear interpolation can approximate the model as $n$ is increasing. Since the generalization error of the linear interpolation has a constant lower bound on the noisy data. Thus, we have the following theorem:

\begin{theorem}[Overfitted network generalizes poorly]\label{thm:bad_gen}
    Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. With the probability at least $1-\frac{2}{n}$, $f_{\infty}^{\NTK}(x)$ can be approximated by the linear interpolation, i.e.,
\begin{align}
 \sup_{x\in [0,1]}|f^{\NTK}_{\infty}(x)-f_{\LI}(x)|\leq C\sqrt{\log(n)} /(n-1)^{2}
\end{align}
for some constant $C$. Moreover, the generalization error of $f_{\infty}^{\NTK}(x)$ is bounded away from zero, i.e.,
    \begin{equation}
       \excrisk(f_{\infty}^{\NTK}) \geq  C
    \end{equation}
 for some constant $C$.
\end{theorem}

\begin{remark}
 To the best of our knowledge, it is the first time to show how wide neural networks interpolate on the data. Combined with Proposition \ref{prop:funct:approx} and Theorem \ref{thm:bad_gen}, our theory shows that for over-fitted neural networks, adding more parameters does not increase the model complexity but makes the models more concise. The experiment results are shown in Figure \ref{fig:LI} (a). That is the reason why over-fitted neural networks can not affect too much by overparameterization.
\end{remark}

\begin{remark}
The second result of Theorem \ref{thm:bad_gen} is to give an example showing that the overfitted neural network can have bad generalization, which contradicts the observation  {\bf (S)}. Since the lower bound $C$ in Theorem \ref{thm:bad_gen} is related to the scale of the noise, we believe the overfitted neural network can not generalize well in most cases unless the noise is small enough. Figure %\ref{fig: d_larger_than_1} (b) gives more examples showing that, even for $d>1$, the generalization error of overfitted networks is bounded away from zero even if the sample size is increasing.
\end{remark}

 Different from RBF kernel (or high order polynomial kernel) ridgeless regression,  Figure \ref{fig:LI} (a) and (b) present that the interpolation ways of the overfitted NTK model $f^{\NTK}_{\infty}(x)$ and wide neural network are nearly linear. Theorem \ref{thm:bad_gen} gives the upper bound of the gap between the overfitted NTK model and the linear interpolation is $O(\frac{1}{n^2})$ while Figure \ref{fig:LI} (c) shows that the gap actually is exactly $O(\frac{1}{n^2})$. These experimental results are in line with the conclusions of Proposition \ref{prop:funct:approx} and Theorem \ref{thm:bad_gen}.

\begin{figure}[htbp]
    \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{NN_with_diff_m.png}
      \centerline{(a)}
  \end{minipage}%
  \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{LI_NTK_RBF.png}
      \centerline{(b)}
  \end{minipage}%
  \begin{minipage}[t]{0.33\linewidth}
      \centering
      \includegraphics[width=\textwidth]{gap_between_NTK_LI.png}
      \centerline{(c)}
  \end{minipage}
  \caption{(a): The interpolation ways of one-hidden-layer neural networks with different widths; (b): The interpolation ways of linear interpolation, $f^{NTK}_{\infty}(x)$ and RBF kernel regression with $\gamma=1$; (c): The gap between $f^{NTK}_{\infty}(x)$ and linear interpolation. The input of the training data is the equally-distanced one-dimensional data $\{x_{i}=\frac{i-1}{n-1}, i \in [n]\}$. The label of the training data is randomly selected from $\{1,-1\}$, which does not contribute to the experiment result. The sample size $n=100,200,...,1000$}\label{fig:LI}
\end{figure}





























\begin{comment}
\subsection{Speculation on $\mathbb{R}^{d}$}

\begin{figure}[htbp]
    \begin{minipage}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\textwidth]{min_eigenvalue_for_diff_d}
        \centerline{(a) Minimum eigenvalue of NTK}
    \end{minipage}%
    \begin{minipage}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\textwidth]{test_error_of_NTK.png}
        \centerline{(b) Generalization error for Overfitted Neural Networks}
    \end{minipage}
    \caption{(a) Minimum eigenvalue of NTK on $\mathbb{R}^{d}$: The input is the equally-distanced data $\{\bm{x}_i\}_{i=1}^n$, defined as $\{(\frac{i_1-1}{n_d-1},...,\frac{i_d-1}{n_d-1})\}$, $i_1,...,i_d\in[n_d]$, where $n_d=n^{\frac{1}{d}}$. We calculate the minimum eigenvalue of NTK with different minimum distances $\frac{1}{n_d-1}$; (b) Generalization error for Overfitted NTK $f^{\NTK}_{\infty}$ over $\mathbb{R}^{d}$: The input $x \sim \unif(0,1)^d$ where $d=2,3,4$. $f_{\star}(x) = \sin(\frac{\sum_{j=1}^{d}x_j}{\sqrt{d}})$ and $y=f_{\star}(x)+0.1\varepsilon$, where $\varepsilon \sim N(0,1)$. The sample size of training data $n=100,300,500,...,1900$ and the number of testing data is $1000$ for all experiments.}
    \label{fig: d_larger_than_1}
  \end{figure}

\subsubsection*{Spectral properties of NTK} The experiment of the minimum eigenvalue is presented in Figure \ref{fig: d_larger_than_1} (a), showing that for fixed $d$, the minimum eigenvalue $\lambda_{\min}$ of $K_d(\bm{X},\bm{X})$ tends to be $\Theta(d_{\min})$, i.e., $c d_{\min}\leq \lambda_{\min} \leq C d_{\min}$ for some constants $c$ and $C$. 

\cite{bietti2019inductive} has shown that on $\mathbb{S}^{d-1}$, the eigenvalues associated with the bias-free NTK $\lambda_k \asymp k^{-\frac{d}{d-1}}$ (considering multiple roots). There are some zero eigenvalues for the bias-free NTK and adding a bias may prevent such zero eigenvalues. Thus, we believe that on $\mathbb{R}^{d}$, the eigenvalues of the NTK with biases $\lambda_k \asymp k^{-\frac{d+1}{d}}$. This conjecture is the key to the generalization ability of neural networks with early stopping.



\subsubsection*{Over-parameterized neural networks are minimax rate optimal with early stopping} We can make the following assumptions:
\begin{assumption}\label{assumption:EDR_for_R_d}
    Let $\lambda_j,j=0,1,2\dots$ be the eigenvalues associated with the NTK $K_d$ defined on $[0,1]^{d}$ and satisfies
\begin{equation}
    \lambda_{j} \asymp j^{-\frac{d+1}{d}}.
\end{equation}
\end{assumption}
\begin{assumption}\label{assumption:f_star_in_H_K_d}
    $f_{\star}\in \mathcal{H}_{K_d}$ where $K_d$ is the NTK.
\end{assumption}
Then with these two assumptions, we have the following results:
\begin{proposition}\label{prop:early:stopping:d} 
Suppose Assumption \ref{assumption:EDR_for_R_d} and \ref{assumption:f_star_in_H_K_d} hold. For the NTK regression, if we stop the training process at  $t_{\star}=\Theta(n^{-(d)/(2d+1)})$, then
\begin{equation}
     \excrisk(f_{t_{\star}}^{\NTK})=O( n^{-(d+1)/(2d+1)}\log^{2}\frac{6}{\delta}),
\end{equation}
with probability at least $1-\delta$ and
\begin{equation}
    \inf_{\hat{f}_{n}}\sup_{f_{\star}\in\mathcal{H}_{K},\lVert f_{\star}\rVert\leq R}\Expc\excrisk(\hat{f}_{n}) =\Omega( n^{-(d+1)/(2d+1)}).
\end{equation}
\end{proposition}
Thus, combined with Theorem \ref{thm:risk:approx}, we show the generalization performance of neural networks with early stopping.


\subsubsection*{Over-fitted neural networks generalize poorly}  The experiment of the generalization error is presented in Figure \ref{fig: d_larger_than_1} (b), showing that for fixed $d$, the generalization error of $f^{\NTK}_{\infty}$ is bounded away from zero even when $n$ is increasing.

In summary, for fixed $d$, the conjectures on the $\mathbb{R}^{d}$ are summarized as followed:

i) Let $\bm{X} = \{\bm{x}_i,...,\bm{x}_n\}\in [0,1]^{d}$ and $d_{\min} = \min_{i\neq j}\|\bm{x}_i-\bm{x}_j\|$. The minimum eigenvalue, $\lambda_{\min}$ of $K_d(\bm{X},\bm{X})$ satisfies 

\begin{equation}
    \lambda_{\min} \asymp d_{\min}
\end{equation}
for some constants $c$, $C$.

ii) Let $\lambda_j,j=0,1,2\dots$ be the eigenvalues associated with the NTK $K_d$ defined on $[0,1]^{d}$ and satisfies
\begin{equation}
    \lambda_{j} \asymp j^{-\frac{d+1}{d}}.
\end{equation}

iii) Assume ii) holds and $f_{\star} \in \mathcal{H}_{K_d}$, then if the width $m$ of the two-layers ReLU neural network is sufficiently large and the training process is stopped at $t_{\star}=\Theta(n^{-(d)/(2d+1)})$, then
    \begin{equation*}
        \excrisk(f_{\bm{\theta}(t_{\star})})=O( n^{-(d+1)/(2d+1)}\log^{2}\frac{6}{\delta}),
    \end{equation*}
    with probability converging to one over initialization and high probability over the training data.

iv) The generalization error of the over-fitted NTK model with zero initialization is bounded away from zero, i.e.,
    \begin{equation}
       \excrisk(f_{\infty}^{\NTK}) \geq  C
    \end{equation}
 for some constant $C$.
\end{comment}




















==> nn_generalization.tex <==
In the following content, we will present the properties of the neural network over one dimensional data $f_{t}^{m}(x)$. For simplicity, let $x\in[0,1]$.  In Section \ref{ntk:recollect}, we have mentioned $f_{t}^{m}$ can be effectively approximated by $f_{t}^{NTK}$. So we will focus on the asymptotic behaviour of $f_{t}^{NTK}(x)$ from now on. The NTK $K(x,x')$ is given by
  \begin{equation}\label{ntk:L=1:d=1}
    K(x,x')= 2\left(1-\psi(x,x')/\pi\right)(x x'+1) +|x-x'| /\pi+1,
\end{equation}
where $\psi(x,x') = \arccos(\frac{xx'+1}{\sqrt{(x^2+1)(x'^2+1)}})\in[0,\frac{\pi}{4}]$.

\subsection{Properties of NTK}\label{subsection:properties_of_ntk} 
In Section \ref{ntk:positive}, we have shown the strictly positive definiteness of NTK. The strictly positive definiteness only guarantees that $\lambda_{n}>0$. We can actually prove a stronger statement.
\begin{lemma}\label{min_eigenvalue} Let $X=\{x_{1},...,x_{n}\}\subset [0,\pi]$ and $d_{min}=\min_{i\neq j}|x_{i}-x_{j}|$. The minimum eigenvalue, $\lambda_{\min}$,  of $K=(K(x_{i},x_{j}))_{1\leq i,j\leq n}$ satisfies that
 \begin{equation}
  \lambda_{\min}\geq \frac{d_{min}}{2\pi}.
  \end{equation}
\end{lemma}
%Add remark how to prove 

The minimum eigenvalue of $K(X_{n},X_{n})$ is of particular interest in understanding the dynamics of the (very) wide neural network. Several groups of researchers studied it for high dimensional data ( e.g., \cite{ghorbani2020neural},\cite{nguyen2021tight}). Most of works implicitly or explicitly assumed that the minimum eigenvalue is a positive constant (\cite{hu2021regularization},\cite{suh2021non}). Lemma \ref{min_eigenvalue} shows that, even for the equally distanced one dimensional data ($d_{min}=\frac{1}{n-1}$), the minimum eigenvalue depends on the sample size. 

\vspace{3mm}

\begin{lemma}\label{lemma:K_decay_rate} 
    Let $\{\lambda_{j}, j=0, 1,2,\cdots\}$ be the eigenvalues associated to the kernel $K$ on $[0,1]$. Then we have 
    \begin{equation}
        \frac{1}{2\pi^3} \frac{1}{j^{2}}\leq \lambda_j \leq \frac{14}{\pi^3} \frac{1}{j^{2}}, j=1,2,...
    \end{equation}
\end{lemma}
%Add remark how to prove 
%\begin{remark}

%\end{remark}
\subsection{Overfitted Neural Network can not generalize well}\label{ntk:linear interpolation}
Since the gradient flow $f_{t}^{m}$ can be effectively approximated by the NTK flow $f_{t}^{NTK}$, we will focus on the asymptotic behaviour of $f_{t}^{NTK}$ from now on. 
%In this subsection we will focus on the 
We are interested in the behaviour of $f^{NTK}_{t}$ when $t$ is sufficiently large. 
To be more concrete, we consider the equally-distanced one dimensional data $\{X_n,Y_n\}=\{(x_{i},y_{i}) \mid x_{i}=\frac{i-1}{n-1}, i \in [n]\}$.
Let 
\begin{align}
    f_{LI}(x)=y_{i}+\frac{y_{i+1}-y_{i}}{x_{i+1}-x_{i}}(x-x_{i}), \mbox{ when } x\in [x_{i},x_{i+1}]
\end{align}
be the linear interpolation of these $n$ points. We can prove the following statement.

\begin{proposition}
[Overfitted NTK model can be approximated by linear interpolation]\label{LI}
Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. The overfitted NTK model with zero initialization $f^{\NTK}_{\infty}(x) =K(\bm{x},\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}$ can be approximated by the linear interpolation, i.e.,
\begin{align}
 \sup_{x\in [0,1]}|f_{\infty}^{\NTK}(x)-f_{LI}(x)|\leq C/(n-1)^{2}
\end{align}
 for some constant $C$.
\end{proposition}

Proposition \ref{LI} implies that a lazy trained overfitted neural network can be approximated by linear interpolation. On the other hand, it is well known that linear interpolation does not generalize well. Thus, we have the following statement.

% Raskutti et al. \cite{raskutti2014early} have considered the regression problem
% \begin{align}\label{equation:true_model}
%     y=f_{\star}(x)+\epsilon, \quad \epsilon\sim N(0,\sigma^{2})
% \end{align}
% where $f_{\star}\in \mathcal{H}_{\Phi}$ is the true model and $\mathcal{H}_{\Phi}$ is the RKHS associated to some kernel $\Phi(\cdot,\cdot)$. 

\begin{theorem}[Overfitted network generalizes poorly]\label{thm:bad_gen}
    Let $\{(x_{i},y_{i})\}$ be the set of $n$ equally-distanced data in $[0,1]$, i.e., $x_i=\frac{i-1}{n-1}$, $i\in [n]$. The error of the overfitted NTK model with zero initialization $f^{NTK}_{\infty}(x) =K(x,X_n)K^{-1}(X_n,X_n)Y_n$ is bounded away from zero, i.e.,
    \begin{equation}
        \Expc\lVert f^{NTK}_{\infty}(x)-f_{\star}(x)\rVert^2 \geq  C
    \end{equation}
 for some constant $C$.
\end{theorem}
Theorem \ref{thm:bad_gen} shows that overfitted network can not generalize well. That means training process should be stopped before the network overfits the data.



\subsection{Wide neural networks are minimax optimal with early stopping}

We have shown in Section \ref{ntk:linear interpolation} that, when the equally-distanced data is fitted, the lazy trained 1-hidden neural network can be approximated by linear interpolation. Thus, a lazy trained overfitted neural network can not generalize well. 

% Raskutti et al. \cite{raskutti2014early}  
Lin et al. \cite{lin2020optimal} have considered the regression problem (Equation \eqref{equation:true_model}). They investigated the generalization ability of the solution obtained by gradient descent method with $0\in \mathcal{H}_{\Phi}$ as the initialization point(function), and showed that a properly chosen early stopping strategy leads to a minimax optimal solution if we know the decay rate of eigenvalues of the kernel. By Lemma \ref{lemma:K_decay_rate}, we have the following theorem  
%It may need more efforts to establish them and will be one of our main focus in future work.

%It is proved in \cite{hu2021regularization} that $\lambda_{i}\asymp i^{-d/(d-1)}$ when the NTK is defined on the sphere $\mathbb{S}^{d-1}$. 

%then it's natural to assume the following
%    for all RKHS restricted to uniform distribution on the sphere, spherical harmonic functions are common basis. The inclusion relations of RKHS only depend on the eigenvalue decay. Faster the decay, larger the RKHS because functions in it are smoother. \cite{lukic2001stochastic} show the necessary and sufficient conditions for draws from a Gaussian process with kernel $\Sigma$ lie in the RKHS of kernel $K$ with probability one are the inclusion operator is Hilbert-Schmidt. We will keep work on proving this assumption in future work. 


% \begin{lemma}[Infinite width linearized neural networks using early stopping are minimax optimal]\label{inf-lin-opt}
%     \[
%         \mathbb{E}\lVert f_{\mathsf{lin},t_{\star}}^{m=\infty,\mathbf{z}}-f_{\star}\rVert_{L^2(\mu)}^2=\mathcal{O}(n^{-2/3})
%     \]
% \end{lemma}


\begin{theorem}[Optimality of early stopping]\label{thm:early:stopping} 
For the overfitted NTK model with zero initialization $f^{\NTK}_{\infty}(x) =K(\bm{x},\bm{X})K^{-1}(\bm{X},\bm{X})\bm{y}$, if we stop the training process at $t_{\star}=c n^{2/3}$, the resulting neural network $f_{t_{\star}}^{\NTK}$ satisfies that
\begin{equation}
     \Expc\lVert f_{t_{\star}}^{\NTK}(x)-f_{\star}\rVert^{2} \leq Cn^{-2/3},
\end{equation}
which matches the minimax lower bounds, since we have
\begin{equation}
    \inf_{\hat{f}}\sup_{f_{\star}\in\mathcal{H}_{K},\lVert f_{\star}\rVert\leq R}\Expc\lVert \hat{f}-f_{\star}\rVert^{2} \geq Cn^{-2/3}.
\end{equation}
\end{theorem}
Combining Theorem \ref{thm:early:stopping} and Proposition \ref{prop: generalization closeness}, Corollary \ref{cor: nn early stopping} follows.
\begin{corollary}\label{cor: nn early stopping}
    If $m>$, then we have
    \begin{equation}
     \Expc\lVert f_{t_{\star}}^{m}(x)-f_{\star}\rVert^{2} \leq Cn^{-2/3},
    \end{equation}
    i.e., the fact that neural network using early stopping is minimax optimal holds with probability at least $1-P(m)$ over random initialization.
\end{corollary}

% $\{\lambda_{i}\geq Ci^{-2}, i=1,2,\cdots\}$ implies that there is a minimax lower bound on the risk  . i.e., For any estimate $\widehat{f}$ of $f_{\star}$ based of the $n$ i.i.d. samples $\{(x_{i},y_{i})\}_{i=1,\cdots,n}$, one has
% \begin{align}
%     \sup_{f_{\star} \in \mathcal{H}_{K}}
%               \int_{0}^{1} ( \widehat{f}-f_{\star})^2 dx \leq C\sigma^{2}n^{-2/3}.
% \end{align}
% In other words, the early stopped $f^{NTK}_{t_{\star}}$ achieves the minimax rate.

The statement that neural network that overfits cannot generalize well seems to contradict the observation (S), however, we realize that it might be caused by the subtle difference between zero training label-error and zero training loss. In other words, we actually stopped earlier than the time we needed to overfit the data. 

We present this subtle difference through the following illustrative example.


\begin{figure}[h]
\centering
\includegraphics[scale=0.4]{100accuracy_vs_interpolation}
\caption{Overfitting vs. 100 \% label accuracy: 4 training data points $\{(0,0),(\frac{1}{3},1),(\frac{2}{3},0), (1,1) \}$. We use gradient descent to train a one-hidden-layer neural network with large width $m=1000$. Compared with the interpolation regime, the loss in the epoch with 100 \% label accuracy is still large. The function in the epoch with 100 \% label accuracy is also far different from the function in the interpolation regime.}
\label{fig: interpolation vs acc}
\end{figure}

\subsection{On the role of signal strength}
Theorem \ref{thm:early:stopping} shows that a carefully chosen early stopping time will produce a neural network  achieving the minimax rate. 
Zhang et al. \cite{zhang2016understanding} observed the implicit early stopping strategy, stopping the training process when the 100\% label accuracy is reached, can generalize well. One may speculate that the implicit early stopping time is the optimal stopping time appeared in Theorem \ref{thm:early:stopping}, however, this sounds too good to be true. In fact, Zhang et al. \cite{zhang2016understanding} have discussed about the role of some explicit early stopping strategies in training the neural networks. They observed that: 1. early stopping indeed make generalization better on ImageNet; and 2. early stopping does not help much on CIFAR10. These observations made the effects of the implicit early stopping elusive. We can not simply claim that implicit early stopping strategy would produce a rate optimal neural network.

We hypothesized that the signal strength plays an indispensable role in the successes of implicit early stopping strategies. More precisely, when the signal strength is strong enough, the implicit early stopping strategy will produce a stopping time near the optimal stopping time $t_{\star}$; and when the signal strength is deteriorated (e.g., after performing some label corruption procedure), the implicit early stopping strategy will produce a stopping time far from the optimal stopping time $t_{\star}$. We give a qualitative analysis the signal strength from two aspects in Section \ref{sec:signal} and answer why overfitted neural networks can generalize on real data. The analysis will be justified in Section \ref{sec:experments} through several experiments including both synthetic data and real data. In summary, we finally filled the last piece of jigsaw in reconciling the controversial observation (S) and the bias-variance trade-off doctrine in classical statistical learning theory.




==> preliminaries.tex <==
\subsection{Settings of the neural networks}

We are interested in analyzing the training process of one-hidden layer neural networks,
\begin{equation*}
  \mathcal{F}^m=\left\{f_{\bm{\theta}}~\middle|~f_{\bm{\theta}}(\bm{x}) = \frac{1}{\sqrt{m}}\sum_{r=1}^{2m} \left(a_{r}\sigma\left(\langle \bm{w}_{r},\bm{x}\rangle+b_{r}\right)\right) + b\right\},
  \end{equation*}
where $\sigma(z) = \max\{z,0\}$ and $\bm{\theta}=\vect(\{a_{r},\bm{w}_{r},b_{r},b,r\in [2m]\})$ is the parameters of the neural network. Initialize the parameters $a_{r}(0),\bm{w}_{r,j}(0),b_{r}(0), b \sim \mathcal{N}(0,1)$ for $r\in [m]$, $j\in [d]$ and set $a_{r+m}(0)=a_{r}(0)$, $\bm{w}_{r+m,j}(0)=\bm{w}_{r,j}(0)$, $b_{r+m}(0)=b_{r}(0)$. Given the
data $\{(\bm{x}_{i},y_{i})\in \mathbb{R}^{d}\times\mathbb{R}, i\in[n]\}$, we are interested in analyzing the gradient flow of the empirical loss function 
\begin{equation*}
    \mathcal{L}_{n}(f_{\bm{\theta}})=\frac{1}{2n}\sum_{i=1}^{n}\left(y_{i}-f_{\bm{\theta}}(\bm{x}_{i})\right)^{2}=\frac{1}{2n}\lVert \bm{y}-f_{\bm{\theta}}(\bm{X})\rVert^{2}
\end{equation*}
where $\bm{X}\in\mathbb{R}^{n\times d}$, $\bm{y}\in\mathbb{R}^{n}$ and $f\in \mathcal{F}^{m}$.

% $\bm{X}=\begin{bmatrix}\bm{x}_{1}\tran \\ \vdots \\ \bm{x}_{n}\tran\end{bmatrix}$

We recollect some well known results in this subsection to make this paper more friendly to the readers.
Let $\bm{\Theta}=\left\{\bm{\theta}~\middle|~ \bm{\theta}\in\mathbb{R}^{(d+2)m+1}\right\}$ be the parameter space of $\mathcal{F}^{m}$. The gradient flow in $\bm{\Theta}$ induced by the loss function is given by
\begin{equation}
\begin{aligned}
      \dot{\bm{\theta}}(t) &=\frac{\dx}{\dx t}\bm{\theta}(t)=-\nabla_{\bm{\theta}}\mathcal{L}_{n}(f_{\bm{\theta}})= - \frac{1}{n}\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})\tran (f_{\bm{\theta}(t)}(\bm{X})-\bm{y})
\end{aligned}
\end{equation}
where $\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})$ is an $n\times ((d+2)m+1)$ matrix.
This flow induced an associated flow in  $\mathcal{F}^{m}$:    
\begin{equation}\label{nn:f:flow}
\begin{aligned} 
\dot{f}_{\bm{\theta}(t)}(\bm{x}) &=\frac{\dx }{\dx t}f_{\bm{\theta}(t)}(\bm{x})=\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{x})\dot{\bm{\theta}}(t)= -\frac{1}{n} K_{\bm{\theta}(t)}(\bm{x},\bm{X}) (f_{\bm{\theta}(t)}(\bm{X})-\bm{y}),
\end{aligned}
\end{equation}
where $K_{\bm{\theta}(t)}(\bm{x},\bm{X}) =\nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{x}) \nabla_{\bm{\theta}} f_{\bm{\theta}(t)}(\bm{X})\tran$. We often refer to $K_{\bm{\theta}(t)}$ as the neural network kernel which is a time-varying kernel. 


\vspace{3mm}

Since Equation \eqref{nn:f:flow} is highly non-linear and hard to find an explicit solution, various approximated solutions (\cite{mei2019mean}, \cite{karakida2019universal}, \cite{sirignano2022mean}, \cite{eldan2021non}) were proposed to characterize the asymptotic behaviour of these equations. In the seminal paper \cite{jacot2018neural}, Jacot et al.  observed that
\begin{align}
    K_{\bm{\theta}(t)}(\bm{x},\bm{x}')\xrightarrow{m\rightarrow \infty} K(\bm{x},\bm{x}')
\end{align}
where $K(\bm{x},\bm{x}')$ is a time independent kernel. This kernel, now often referred to as the neural tangent kernel (NTK), leads us to consider the following gradient flow
\begin{equation}\label{ntk:f:flow}
    \begin{aligned}
    \dot{f}^{\NTK}_{t}(\bm{x})=\frac{\dx}{\dx t}f^{\NTK}_{t}(\bm{x})=-\frac{1}{n}K(\bm{x},\bm{X})(f^{\NTK}_{t}(\bm{X})-\bm{y})
    \end{aligned}
\end{equation}
in the space $\mathcal{F}$, the reproducing kernel Hilbert space (RKHS) associated to the kernel $K$. $K(\bm{x},\bm{X}) = (K(\bm{x},\bm{x}_1),\dots,K(\bm{x},\bm{x}_n))\in \mathbb{R}^{1\times n}$. Similar to the neural network function, we assume $f^{\NTK}_{t}(\bm{x})=0$.

Though it is hard to analyze the solution $f_{\bm{\theta}(t)}$ of the equation \eqref{nn:f:flow} directly, we may focus on the solution $f^{\NTK}_{t}$ of the equation \eqref{ntk:f:flow} first if $m$ is sufficiently large. This simplifies the problem substantially, as we can solve the equation \eqref{ntk:f:flow}  explicitly: 
\begin{equation}\label{ntk:solution}
    f_t^{\NTK}(\bm{x})=K(\bm{x},\bm{X})K(\bm{X},\bm{X})^{-1}(\bm{I}-e^{-\frac{1}{n}K(\bm{X},\bm{X})t})\bm{y}
\end{equation}

\subsection{Uniform NTK Approximation for Wide Neural Networks}\label{subsec: unif ntk approx}

One may naturally expect that the solution $f_{\bm{\theta}(t)}$ of the equation \eqref{nn:f:flow} and the solution $f^{\NTK}_{t}$ of the equation \eqref{ntk:f:flow} should behave in a similar way for sufficiently large $m$.  
Furthermore, when $m$ is sufficiently large, 
some researchers often referred to the flow $f_{\bm{\theta}(t)}$ as the lazy trained neural network, for 
the movement of $\bm{\theta}(t)$ is ignorable in this scenario (e.g., \cite{lee2019wide},\cite{du2018gradient},\cite{jacot2018neural}).
These statements have been justified in a sequence of works from various groups of researchers (see e.g., \cite{jacot2018neural},\cite{arora2019exact},\cite{lee2019wide}). 

% comparisons with other similar work
We are aware of that \cite{hu2021regularization}, \cite{suh2022nonparametric} have shown that the generalization error of the neural network trained for too long is bounded away from zero. However, it is worth noting that both of their results need NTK regression as a intermediate term. Then it is necessary to prove that the generalization error of the neural network could be approximated by that of NTK regression. Since the generalization error is related to all $\bm{x}$, the uniform convergence of the difference between the output of the neural network and that of NTK regression, i.e., $\sup_{\bm{x}}\abs{f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})}=o_{m}(1)$. Notice that \eqref{nn:f:flow} and \eqref{ntk:f:flow} indicate the evolution of $f_{\bm{\theta}(t)}$ and $f_{t}^{\NTK}$ is fully determined by their kernel $K_{\bm{\theta}(t)}$ and $K$ respectively, it is important to give the uniform convergence of the difference between the two kernel, i.e., $\sup_{\bm{x},\bm{x}'}\abs{K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K(\bm{x},\bm{x}')}=o_{m}(1)$. To the best of our knowledge, we give the first concrete result on that the generalization error of the fully trained two-layers ReLU neural networks could be represented by NTK regression, which is our Proposition \ref{prop: generalization closeness}. 

% fill the gap that the generalization ability of the wide neural network can be approximated by the NTK regression. A lot of work use the generalization ability of NTK to represent the neural network(see ). to the best of our knowledge, there is no work showing this, which need the uniform approximation of NTK to the kernel of neural network at training of finite width. Previous studies of the NTK have not dealt with the uniform convergence of kernel, which is necessary for claiming the generalization ability approximation. Here, we need to emphasize the proof from \cite{du2018gradient} can only prove point-wise convergence.

\begin{theorem}\label{thm: kernel closeness}
    Assume that $\lambda_{\min}(K(\bm{X},\bm{X}))>0$. If $m$ is sufficiently large(depending on $\lambda_{\min}(K(\bm{X},\bm{X}))$), then
    \begin{equation*}
    \Prob_{\bm{\theta}(0)}\left(\sup_{\bm{x},\bm{x}'}\sup_{t\geq 0}\left\lvert K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K(\bm{x},\bm{x}')\right\rvert\leq cm^{-(1-\gamma)}\log m\right)\geq 1-P(m),
    \end{equation*}
    where $P(m)\to 0$ as $m\to\infty$.
\end{theorem}

The important assumption on $\lambda_{\min}(K(\bm{X},\bm{X}))$ will be proven in the next subsection.

Results from previous work (refs) could be summarized as the point-wise convergence of kernel. The problem is that although each point-wise convergence holds with high probability, there is no grantee on the uniform convergence with high probability using the union bound. More delicate analysis is needed.

% We have to emphasize that Theorem \ref{thm: kernel closeness} holds for the ReLU activation function while the existing similar results (e.g., \cite{du2019gradient} \cite{lee2019wide}) all required that the activation functions have bounded second derivatives and this is the first result showing uniform kernel approximation. We will discuss two important assumptions. We will prove $\lambda_{\min}(K(\bm{X},\bm{X}))$ in the next subsection.

% Since the ..., we here give the main ingredients for proving Theorem \ref{thm: kernel closeness}.

For brevity, denote the pre-activation value and the activation pattern for the $r$-th neuron by $h_{\bm{\theta}}^{r}(\bm{x})=\langle \bm{w}_{r},\bm{x}\rangle+b_{r}$ and $\bm{1}_{\bm{\theta}}^{r}(\bm{x})=\bm{1}_{\{h_{\bm{\theta}}^{r}(\bm{x})\geq 0\}}$ respectively.

Lemma \ref{lem: event B}, Lemma \ref{lem: event C} and Lemma \ref{lem: event R} are the building blocks to prove Theorem \ref{thm: kernel closeness}. Proofs are left in Appendix \ref{app: unif ntk approx}.

Check
\begin{itemize}
    \item $\alpha<1/2$
    \item $1-\gamma<\beta/2$
    \item $\gamma>\max\{1-\alpha,\delta\}$
    \item $\beta>\alpha$
\end{itemize}

\begin{lemma}\label{lem: event B}
    Define the event 
    \begin{equation*}
        \mathcal{B}=\left\{\omega\mid \lvert a_{r}(0)\rvert,\lvert \bm{w}_{r,j}(0)\rvert,\lvert b_{r}(0)\rvert\leq R_{B}, r\in[2m], j\in[d]\right\}, \text{~where~} R_{B}=\sqrt{3 \log m}.
    \end{equation*}
    Conditioning on the event $\mathcal{B}$, we have $\lvert h_{\bm{\theta}(0)}^{r}(\bm{x})\rvert\leq cR_{B}$ for all $r\in [2m]$ and $\bm{x}$. The event $\mathcal{B}$ holds with high probability, i.e., $\Prob_{\bm{\theta}(0)}(\mathcal{B})\geq 1-P_{\mathcal{B}}(m)$, where $P_{\mathcal{B}}(m)=cm^{-1/2}$.
\end{lemma}

\begin{remark}
    Lemma \ref{lem: event B} control the scale of the parameters of the neural network at initialization.
\end{remark}

Our main contribution is the uniform convergence of kernel which relies on the analysis the continuity of $K_{\bm{\theta}(0)}$ and $K$ when the domain $\mathcal{X}$ is discretized. On each dimension, we place $\lceil m^{\beta}\rceil$ points with distance $\epsilon=B/\lceil m^{\beta}\rceil$. Denote the collection $\mathcal{N}_{\epsilon}$ so that $\lvert\mathcal{N}_{\epsilon}\rvert=\lceil m^{\beta}\rceil^{d}$. The idea is to use $\mathcal{N}_{\epsilon}$ to discretize the domain $\mathcal{X}$ and then use classical concentration inequality on points in $\mathcal{N}_{\epsilon}$, which gives probability decaying exponentially fast with $m$. We need the following three lemmas to show events we need to condition on hold with probability converging to one as $m\to\infty$. 

\begin{lemma}\label{lem: event R}
    Define the events 
    \begin{gather*}
        \mathcal{R}(\mathcal{N}_{\epsilon})=\left\{\omega ~\middle|~ \abs{h_{\bm{\theta}(0)}^{r}(\bm{z})}> 2cR\mbox{~holds for at least~}2(m-\lceil m^{\gamma}\rceil)\mbox{~of~} r \in [2m],\forall\bm{z}\in\mathcal{N}_{\epsilon}\right\}\\
    \text{and~}\mathcal{R}=\left\{\omega ~\middle|~ \abs{h_{\bm{\theta}(0)}^{r}(\bm{x})}> cR\mbox{~holds for at least~}2(m-\lceil m^{\gamma}\rceil)\mbox{~of~} r\in [2m],\forall\bm{x}\right\},
    \end{gather*}
    where $R=cm^{-\alpha}$. If $m$ is sufficiently large, then $\mathcal{R}\supseteq\mathcal{R}(\mathcal{N}_{\epsilon})$ and the event $\mathcal{R}$ holds with high probability, i.e., $\Prob_{\bm{\theta}(0)}\left(\mathcal{R}\right)\geq \Prob_{\bm{\theta}(0)}\left(\mathcal{R}(\mathcal{N}_{\epsilon})\right)\geq 1-P_{\mathcal{R}}(m)$, where $P_{\mathcal{R}}(m)=\lceil m^{\beta}\rceil^{d}e^{-2m^{2\delta-1}}$.
\end{lemma}

\begin{remark}
    Lemma \ref{lem: event R} shows the pre-activation value of most neurons are large, which hints that the activation pattern for these neurons is likely to stay unchanged during training since large pre-activation value requires the parameters to travel a long way from the initialization to make the sign change. This is crucial to prove lazy.
\end{remark}

\begin{lemma}\label{lem: event C}
    Define the event 
    \begin{equation*}
        \mathcal{C}=\left\{\omega ~\middle|~ \sup_{\bm{z},\bm{z}'\in\mathcal{N}_{\epsilon}}\lvert K_{\bm{\theta}(0)}(\bm{z},\bm{z}')-K(\bm{z},\bm{z}')\rvert\leq cm^{-1/2}\sqrt{\log m}\right\}.
    \end{equation*}
    If $m$ is sufficiently large, then the event $\mathcal{C}$ holds with high probability, i.e., $\Prob_{\bm{\theta}(0)}\left(\mathcal{C}\right)\geq 1-P_{\mathcal{C}}(m)$, where $P_{\mathcal{C}}(m)=4m^{-(c_{0}c^{2}/c_{B}-2d\beta)}$, where $c_{0}$ is a absolute constant and $c_{B}$ is a constant depending on $B$.
\end{lemma}

\begin{remark}
    It is intuitive that the point-wise convergence of $K_{\bm{\theta}(0)}-K$ holds simply by the law of large numbers. The result from Lemma \ref{lem: event C} shows this convergence is uniform for points in the collection $\mathcal{N}_{\epsilon}$.
\end{remark}

To prove Theorem \ref{thm: kernel closeness}, we only need Lemma \ref{lem: initial kernel close to fixed} and Lemma \ref{lem: kernel with lazy params close to initial kernel} to show that the convergence of kernel at the initialization and during training, and then use the triangle inequality $\abs{K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K(\bm{x},\bm{x}')}\leq\abs{K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K_{\bm{\theta}(0)}(\bm{x},\bm{x}')}+\abs{K_{\bm{\theta}(0)}(\bm{x},\bm{x}')-K(\bm{x},\bm{x}')}$. The proof of Lemma \ref{lem: initial kernel close to fixed} and Lemma \ref{lem: kernel with lazy params close to initial kernel} could be found in Appendix \ref{app: unif ntk approx}.

\begin{lemma}\label{lem: initial kernel close to fixed}
    Conditioning on the event $\mathcal{B}\cap\mathcal{R}\cap\mathcal{C}$, if $m$ is sufficiently large, then
    \begin{equation*}
        \sup_{\bm{x},\bm{x}}\lvert K_{\bm{\theta}(0)}(\bm{x},\bm{x}')-K(\bm{x},\bm{x}')\rvert\leq cm^{-(1-\gamma)}\log m.
    \end{equation*}
\end{lemma}

\begin{remark}
    Notice that Lemma \ref{lem: initial kernel close to fixed} is an extension of Lemma \ref{lem: event C}. The key reason why Lemma \ref{lem: initial kernel close to fixed} is true is due to the continuity of $K_{\bm{\theta}(0)}$ and $K$.
\end{remark}

\begin{lemma}\label{lem: kernel with lazy params close to initial kernel}
    Assume that $\lambda_{\min}(K(\bm{X},\bm{X}))>0$. Conditioning on the event $\mathcal{B}\cap\mathcal{R}\cap\mathcal{C}$, if $m$ is sufficiently large(depending on $n,\lambda_{\min}(K(\bm{X},\bm{X})),...$),then
    \begin{equation*}
        \sup_{\bm{x},\bm{x}'}\sup_{t\geq 0}\lvert K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K_{\bm{\theta}(0)}(\bm{x},\bm{x}')\rvert\leq cm^{-(1-\gamma)}\log m.
    \end{equation*}      
\end{lemma}

\begin{remark}
    The continuity of $K_{\bm{\theta}}$ w.r.t. $\bm{\theta}$.
\end{remark}

Using Theorem \ref{thm: kernel closeness}, we can further prove the uniform function approximation as follows, whose proof is deferred in Appendix \ref{app: unif ntk approx}. 

\begin{proposition}\label{prop: function closeness}
    Assume that $\lambda_{\min}(K(\bm{X},\bm{X}))>0$. If $m$ is sufficiently large(depending on $\lambda_{\min}(K(\bm{X},\bm{X}))$), then
    \begin{equation*}
        \Prob_{\bm{\theta}(0)}\left(\sup_{\bm{x}}\sup_{t\geq 0}\lvert f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})\rvert\leq cm^{-(1-\gamma)}\log m\right)\geq 1-P(m).
    \end{equation*}    
\end{proposition}

Thanks to the uniform function approximation, we now can formally show that the test performance of wide neural networks can be represented by NTK regression.

\begin{proposition}\label{prop: generalization closeness}
    Assume that $\lambda_{\min}(K(\bm{X},\bm{X}))>0$. Given the training data, if $m$ is sufficiently large, then
    \begin{equation*}
        \abs{\lVert f_{\bm{\theta}(t)}-f_{\star}\rVert^{2}-\lVert f_{t}^{\NTK}-f_{\star}\rVert^{2}}\leq cm^{-(1-\gamma)}\log m    
    \end{equation*}
    holds with probability at least $1-P(m)$ w.r.t. the initialization and with probability at least $1-\delta$ w.r.t. the training data.
\end{proposition}

\begin{proof}
    \begin{equation*}
        \begin{aligned}
            & \lVert f_{\bm{\theta}(t)}-f_{\star}\rVert^{2}-\lVert f_{t}^{\NTK}-f_{\star}\rVert^{2}\\ 
            =&\int_{\mathcal{X}}(f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})+2(f_{t}^{\NTK}(\bm{x})-f_{\star}(\bm{x})))(f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x}))\dx \mu(\bm{x})\\
            \leq &c\sup_{\bm{x}}\sup_{t\geq 0}\lvert f_{\bm{\theta}(t)}(\bm{x})-f_{t}^{\NTK}(\bm{x})\rvert
        \end{aligned}    
    \end{equation*}
\end{proof}

In the next subsection, we will discuss strictly positive definiteness of NTK $K$ over $\mathbb{R}^{d}$.

\subsection{Strictly positive definiteness of NTK over $\mathbb{R}^{d}$}\label{ntk:positive}
To avoid the potential confusions between positive definiteness and semi-positive definiteness, we introduce the notion of strictly positive definiteness below. 
\begin{definition}
       A kernel $K$ is strictly positive definite over domain $\mathcal{X}\subset \mathbb{R}^{d}$ if for any $n$ and any points $\bm{x}_{1},\dots,\bm{x}_{n}\in \mathcal{X}$, the smallest eigenvalue $\lambda_{\min}$ of the matrix $(K(\bm{x}_{i},\bm{x}_{j}))_{1\leq i,j\leq n}$ is larger than zero.
\end{definition}

We have to emphasize that in order to make the neural tangent approximation hold, we need to know that $K$, the neural tangent kernel, is strictly positive definite on its domain.  This has been only proved for NTKs defined on $\mathbb{S}^{d-1}$ (\cite{jacot2018neural}). If the neural tangent kernel $K$ is strictly positive definite, then one can easily see that the gradient flow $f^{\NTK}_{t}$  in $\mathcal{F}$ will achieve the global minima. As a direct corollary, for sufficiently large $m$, the gradient flow $f_{\bm{\theta}(t)}$ in $\mathcal{F}^{m}$ will achieve the global minima with high probability.

Combining the results in \cite{cho2009kernel}  and \cite{jacot2018neural}, we can get the following  explicit expression for the neural tangent kernel:

\begin{equation}
\begin{split}
    K(\bm{x},\bm{x}') &= 2\left(1-\psi(\bm{x},\bm{x}')/\pi\right)(\langle \bm{x},\bm{x}' \rangle +1) \\
    &+ \sqrt{\lVert\bm{x} - \bm{x}'\rVert^2_2 + \lVert \bm{x} \rVert^2_2 \lVert \bm{x}' \rVert^2_2 - \langle \bm{x},\bm{x}'\rangle^2 }/\pi + 1,
\end{split}
\end{equation}
where $\psi(\bm{x},\bm{x}')=\arccos$\resizebox{!}{0.3cm}{$\frac{ \langle \bm{x},\bm{x}' \rangle+1}{\sqrt{ (\lVert \bm{x}\rVert^2_2 +1)(\lVert \bm{x}'\rVert^2_2 +1)}}$}.

%Jacot et al. \cite{jacot2018neural} have shown that $K$ is strictly positive definite when it is restricted on the sphere $\mathbb{S}^{d-1}$. 
One of the most important observations in this study is the following: 
\begin{theorem} \label{PD}
    The neural tangent kernel $K(\bm{x},\bm{x}')$ is strictly positive definite on $\mathbb{R}^{d}$.
\end{theorem}
\begin{remark}
The idea of Theorem \ref{PD} is based on the fact that the inner-product kernel determined by the non-polynomial function is strictly positive definite on $\mathbb{S}^{d}_+ :=\{\bm{x}=(x_1,...,x_{d+1})\in \mathbb{S}^{d+1}\mid x_{d+1}>0\}$.
\end{remark}



We have shown the strictly positive definiteness of NTK. The strictly positive definiteness only guarantees that $\lambda_{\min}>0$. However, the minimum eigenvalue can be related to the sample size $n$(the minimum distance), shown in Figure \ref{fig:min_eigenvalue}. For example, we can actually prove a stronger statement over data of dimension one.
\begin{lemma}\label{min_eigenvalue} Let $X=\{x_{1},...,x_{n}\}\subset [0,\pi]$ and $d_{\min}=\min_{i\neq j}|x_{i}-x_{j}|$. The minimum eigenvalue, $\lambda_{\min}$,  of $K=(K(x_{i},x_{j}))_{1\leq i,j\leq n}$ satisfies that
 \begin{equation}
  \lambda_{\min}\geq \frac{d_{\min}}{2\pi}.
  \end{equation}
\end{lemma}

\begin{remark}
The minimum eigenvalue of $K(X_{n},X_{n})$ is of particular interest in understanding the dynamics of the (very) wide neural network. Several groups of researchers studied it for high dimensional data ( e.g., \cite{ghorbani2020neural},\cite{nguyen2021tight}). Most of works implicitly or explicitly assumed that the minimum eigenvalue is a positive constant (\cite{hu2021regularization},\cite{suh2021non}). Lemma \ref{min_eigenvalue} shows that, for the asymptotic analysis, the minimum eigenvalue depends on the sample size $n$. For example, for the equally distanced one dimensional data, the minimum distance $d_{\min}=\frac{1}{n-1}$ and the result is shown in Figure \ref{fig:min_eigenvalue} (a). And we find that for $d>1$, the minimum eigenvalue also depends on the the minimum distance, shown in Figure  \ref{fig:min_eigenvalue}.
\end{remark}

\begin{corollary}\label{cor: kernel closeness}
If $m$ is sufficiently large(depending on $\lambda_{\min}(K(\bm{X},\bm{X}))$), then
    \begin{equation*}
    \Prob_{\bm{\theta}(0)}\left(\sup_{\bm{x},\bm{x}'}\sup_{t\geq 0}\left\lvert K_{\bm{\theta}(t)}(\bm{x},\bm{x}')-K(\bm{x},\bm{x}')\right\rvert\leq cm^{-(1-\gamma)}\log m\right)\geq 1-P(m),
    \end{equation*}
    where $P(m)\to 0$ as $m\to\infty$.
\end{corollary}

\begin{figure}[htbp]
  \begin{minipage}[t]{0.5\linewidth}
      \centering
      \includegraphics[width=\textwidth]{min_eigenvalue_d_1.png}
      \centerline{(a) $\lambda_{min}$ for the equally distanced data(d=1)}
  \end{minipage}%
  \begin{minipage}[t]{0.5\linewidth}
      \centering
      \includegraphics[width=\textwidth]{min_eigenvalue_for_diff_d.png}
      \centerline{(b) $\lambda_{min}$ for the equally distanced data(d>1)}
  \end{minipage}
  \caption{Minimum eigenvalue vs sample size(the minimum distance). (a) Let $\{x_i\}_{i=1}^n$ be the n equally-distanced one dimensional data in [0,1], i.e., $x_i=\frac{i-1}{n-1}$ for $i\in[n]$. We calculate the minimum eigenvalue of NTK with different sample size $n$. (b) For $d>1$, the equally-distanced data $\{\bm{x}_i\}_{i=1}^n$ is defined as $\{(\frac{i_1-1}{n_d-1},...,\frac{i_d-1}{n_d-1})\}$, $i_1,...,i_d\in[n_d]$, where $n_d=n^{\frac{1}{d}}$. We calculate the minimum eigenvalue of NTK with different minimum distances $\frac{1}{n_d-1}$.}%Add some comments
  \label{fig:min_eigenvalue}
\end{figure}


==> proofs.tex <==
\subsection{Proofs of Section \ref{subsec: unif ntk approx}}

%Uniform NTK approximation for wide NN

For brevity, let $h_{\boldsymbol{x}}^{r}=\langle \boldsymbol{w}_{r},\boldsymbol{x}\rangle+b_{r}$, $\mathbf{1}_{\boldsymbol{x}}^{r}=\mathbf{1}_{\{h_{\boldsymbol{x}}^{r}\geq 0\}}$, $\mathbf{1}_{\boldsymbol{x}\boldsymbol{x}'}^{r}=\mathbf{1}_{\{h_{\boldsymbol{x}}^{r}\geq 0,h_{\boldsymbol{x}'}^{r}\geq 0\}}$ and $h_{\boldsymbol{x}}^{r}(t),\mathbf{1}_{\boldsymbol{x}}^{r}(t),\mathbf{1}_{\boldsymbol{x}\boldsymbol{x}'}^{r}(t)$ represent those at time $t$. To start with, we control the parameters at initialization.

\begin{lemma}\label{lem: event B}
    Define the event 
    \begin{equation*}
        \mathcal{B}=\left\{\omega\mid \lvert a_{r}(0)\rvert,\lvert \boldsymbol{w}_{r,j}(0)\rvert,\lvert b_{r}(0)\rvert\leq R_{B}, r\in[2m], j\in[d]\right\}, \text{~where~} R_{B}=\sqrt{3 \log m}.
    \end{equation*}
    Conditioning on the event $\mathcal{B}$, we have $\lvert h_{\boldsymbol{x}}^{r}(0)\rvert\leq (dB+1)R_{B}$ for all $r\in [2m]$ and $\boldsymbol{x}$. The event $\mathcal{B}$ holds with high probability, i.e., $\Prob_{\bm{\theta}(0)}(\mathcal{B})\geq 1-P_{\mathcal{B}}(m)$, where $P_{\mathcal{B}}(m)=\frac{2(d+2)}{\sqrt{2\pi}}m^{-1/2}$.
\end{lemma}

Our main contribution is the uniform. On each dimension, we place $\lceil m^{\beta}\rceil$ points with distance $\epsilon=B/\lceil m^{\beta}\rceil$, where $\beta>0$ to be determined later. Denote the collection $\mathcal{N}_{\epsilon}$ so that $\lvert\mathcal{N}_{\epsilon}\rvert=\lceil m^{\beta}\rceil^{d}$. The idea is to use $\mathcal{N}_{\epsilon}$ to discretize the domain $\mathcal{X}$ and then use classical concentration inequality on points in $\mathcal{N}_{\epsilon}$, which gives probability decaying exponentially fast with $m$. We need the following three lemmas to show events we need to condition on hold with probability converging to one as $m\to\infty$. 


\begin{lemma}\label{lem: event R}
    Define the events 
    \begin{gather*}
        \mathcal{R}(\mathcal{N}_{\epsilon})=\left\{\omega ~\middle|~ \lvert h_{\boldsymbol{z}}^{r}(0)\rvert> 2(d^{1/2}B+1)R\mbox{~holds for at least~}m-\lceil m^{\gamma}\rceil\mbox{~of~} r \in [m],\forall\boldsymbol{z}\in\mathcal{N}_{\epsilon}\right\}\\
    \text{and~}\mathcal{R}=\left\{\omega ~\middle|~ \lvert h_{\boldsymbol{x}}^{r}(0)\rvert> (d^{1/2}B+1)R\mbox{~holds for at least~}m-\lceil m^{\gamma}\rceil\mbox{~of~} r\in [m],\forall\boldsymbol{x}\right\},
    \end{gather*}
    where $R=\frac{\sqrt{2\pi}}{4(d^{1/2}B+1)}m^{-\alpha}$. If $m$ is sufficiently large than a constant depending on $d,B,\alpha,\beta,\gamma,\delta$, $\gamma>\max\{1-\alpha,\delta\}$, and $\beta>\alpha$, then we have $\mathcal{R}\supseteq\mathcal{R}(\mathcal{N}_{\epsilon})$ and the event $\mathcal{R}$ holds with high probability, i.e., $\Prob_{\bm{\theta}(0)}\left(\mathcal{R}\right)\geq \Prob_{\bm{\theta}(0)}\left(\mathcal{R}(\mathcal{N}_{\epsilon})\right)\geq 1-P_{\mathcal{R}}(m)$, where $P_{\mathcal{R}}(m)=\lceil m^{\beta}\rceil^{d}e^{-2m^{2\delta-1}}$.
\end{lemma}


\begin{lemma}\label{lem: event C}
    Define the event 
    \begin{equation*}
        \mathcal{C}=\left\{\omega ~\middle|~ \sup_{\boldsymbol{z},\boldsymbol{z}'\in\mathcal{N}_{\epsilon}}\lvert K_{\bm{\theta}(0)}(\boldsymbol{z},\boldsymbol{z}')-K(\boldsymbol{z},\boldsymbol{z}')\rvert\leq c\frac{\log m}{\sqrt{m}}\right\}.
    \end{equation*}
    The event $\mathcal{C}$ holds with high probability, i.e., $\Prob_{\bm{\theta}(0)}\left(\mathcal{C}\right)\geq 1-P_{\mathcal{C}}(m)$
\end{lemma}

We only need the following two lemmas to show at initialization and during training, and then triangle inequality to prove Proposition \ref{prop: kernel closeness}.

\begin{lemma}\label{lem: initial kernel close to fixed}
    Conditioning on  $\mathcal{B}\cap\mathcal{R}\cap\mathcal{C}$, we have
    \begin{equation}
        \sup_{\boldsymbol{x},\boldsymbol{x}}\lvert K_{\bm{\theta}(0)}(\boldsymbol{x},\boldsymbol{x}')-K(\boldsymbol{x},\boldsymbol{x}')\rvert\leq \frac{1}{m^{1-\gamma}}R_{B}^{2}.
    \end{equation}    
\end{lemma}

\begin{lemma}\label{lem: kernel with lazy params close to initial kernel}
    Conditioning on  $\mathcal{B}\cap\mathcal{R}$, we have
    \begin{equation}
        \sup_{\boldsymbol{x},\boldsymbol{x}'}\sup_{t\geq 0}\lvert K_{t}^{m}(\boldsymbol{x},\boldsymbol{x}')-K_{\bm{\theta}(0)}(\boldsymbol{x},\boldsymbol{x}')\rvert\leq \frac{1}{m^{1-\gamma}}.
    \end{equation}      
\end{lemma}

\subsection{Proofs of Section \ref{ntk:positive}}
%PD of NTK
The proof of Theorem \ref{PD} is based on the strictly positive definiteness on $\mathbb{S}^d$.
\begin{proof}[Proof of Theorem \ref{PD}]
 
Let $\bm{z}^{\top}=(\bm{x}^{\top},1)$. We then have
\begin{align*}
        K(\bm{x},\bm{x}') &= (\left<\bm{x},\bm{x}'\right>+1) \kappa_0(\bm{z},\bm{z}') +\kappa_1(\bm{z},\bm{z}')+ 1\\
    &=\left<\bm{x},\bm{x}'\right> \kappa_0(\bm{z},\bm{z}') + 1 +\kappa_1(\bm{z},\bm{z}')+\kappa_{0}(\bm{z},\bm{z}')
\end{align*}
where $
\kappa_{n}(\bm{z},\bm{z}^\prime):=2\mathbb{E}_{\omega\sim \mathcal{N}(0,I)}[\sigma(\omega\cdot \bm{z})\sigma(\omega\cdot \bm{z}^\prime)(\omega\cdot \bm{z})^{n}(\omega\cdot \bm{z}^\prime)^{n}]$
and $\sigma(x):=max(x,0)$. 

\cite{cho2009kernel} showed that 
\begin{equation}
    \kappa_{n}(\bm{z},\bm{z}')=\lVert \bm{z}\rVert^{n}\lVert \bm{z}'\rVert^{n}J_{n}\left(\frac{\bm{z}}{\lVert \bm{z}\rVert},\frac{\bm{z}'}{\lVert \bm{z}'\rVert}\right)
\end{equation}
where $J_{n}$ defined on $\mathbb{S}^{(d-1)}\times \mathbb{S}^{(d-1)}$ only depends  on the angle $\theta=\arccos\left(\frac{\bm{z}\cdot \bm{z}^\prime}{\lVert \bm{z}\rVert\lVert \bm{z}^\prime\rVert}\right)$. 

We only need to prove that for distint $n$ points $x_{1},\cdots,x_{n}\in \mathbb{R}^{d}$, the matrix $K_{n}=(K(x_{i},x_{j}))_{1\leq i,j\leq n}$ is the strictly positive definite matrix. Since $\|\bm{z}_{i}\|\geq 1$, $i=1,2,\cdots,n$, we have
\begin{align}
    &\lambda_{\min}((\kappa_{1}(\bm{z}_{i},\bm{z}_{j}))_{1\leq i,j\leq n})\geq     \lambda_{\min}((J_{1}(\bm{z}_{i}/\|\bm{z}_{i}\|,\bm{z}_{j}/\|\bm{z}_{j}\|))_{1\leq i,j\leq n}).
\end{align}
On the other hand, we have
\begin{align}
      \lambda_{\min}((\kappa_{0}(\bm{z}_{i},\bm{z}_{j}))_{1\leq i,j\leq n})\geq     \lambda_{\min}((J_{0}(\bm{z}_{i}/\|\bm{z}_{i}\|,\bm{z}_{j}/\|\bm{z}_{j}\|))_{1\leq i,j\leq n}).  
\end{align}
Since \cite{jacot2018neural} showed that $J_{0}+J_{1}$ is strictly positive definite on $\mathbb{S}^{d}$, we know that
\begin{align}
    \lambda_{\min}(K_{n})\geq       \lambda_{\min}((\kappa_{1}(\bm{z}_{i},\bm{z}_{j}))_{1\leq i,j\leq n})+\lambda_{\min}((\kappa_{0}(\bm{z}_{i},\bm{z}_{j}))_{1\leq i,j\leq n})>0 
\end{align}
as $\bm{z}_{i}/\|\bm{z}_{i}\|$ are distinct points in $\mathbb{S}^{d}$. 
\end{proof}


%------------Proofs of Section 3------------------

%Linear interpolation
The proof of Theorem \ref{thm:bad_gen} is based on Proposition \ref{LI} since Proposition\ref{LI} shows that $f_{\infty}^{NTK}$ is close to the linear interpolation. Thus, the proof of Proposition \ref{LI} is the key step and also shown in the following content.

Before we prove Proposition \ref{LI}, we need the following lemma:
\begin{lemma}\label{lemma:K_second_derivative_K_inv}
    Suppose that $n>22$.  There exits a constant $C$ such that for any $1\leq i \leq n-1$ and any $\xi_{i} \in(x_i,x_{i+1})$, 
    \begin{equation}\label{eqn:ess:bound}
    \left|\left(K^{''}(\xi,X_n)K^{-1}\right)_{j}\right| \leq 
    \begin{cases}
    \quad      C &   j\in\{1,i,i+1,n\},\\
    \quad      \frac{C}{n-1}  &  j\not \in \{ 1,i,i+1,n\}.
    \end{cases}
    \end{equation}
    \end{lemma}

The idea of Lemma \ref{lemma:K_second_derivative_K_inv} is to show the second term of Taylor Expansion of $f_{\infty}^{NTK}$ is ignorable as $n$ is large enough. That is the reason why $f_{\infty}^{NTK}$ can be approximated by the linear interpolation.

\begin{proof}[Proof of Proposition \ref{LI}]
    Since 
    \begin{equation*}
         y_{i} = K(x_i,X_n)K^{-1}Y_n
    \end{equation*}
and 
\begin{equation*}
         y_{i+1} = K(x_{i+1},X_n)K^{-1}Y_n,
    \end{equation*}
the Taylor Expansion and intermediate theorem imply that for $\forall x\in(x_{i},x_{i+1})$, there are $\xi_{i}$ and $\hat{\xi}_{i}\in (x_{i},x_{i+1})$ such that 
\begin{align}\label{equation:taylor_expansion}
 K(x,X_n)K^{-1}Y_n -y_{i}&= (x-x_i)K_{+}^{'}(x_i,X_n)K^{-1}Y_n + \frac{(x-x_i)^2}{2}K^{''}(\xi_i,X_n) K^{-1}Y_n,\\
     y_{i+1}-y_{i}%&= (K(x_{i+1},X_n)-K(x_i,X_n))K^{-1}Y_n\\
    &=(x_{i+1}-x_i)K_{+}^{'}(x_i,X_n)K^{-1}Y_n + \frac{(x_{i+1}-x_i)^2}{2}K^{''}(\hat{\xi}_i,X_n)K^{-1}Y_n
\end{align}
 where 
$K^{'}_{+}(x_{i},X_n)=\lim_{x\rightarrow x_{i}^{+}} K^{'}_{+}(x,X_n) = \lim_{x\rightarrow x_{i}^{+}}\frac{\partial K(x,X_n)}{\partial x}$. Thus,
\begin{equation}
\begin{aligned}\label{eq:higher:order}
    K(x,X_n)K^{-1}Y_n& - y_i - \frac{(x-x_i)}{x_{i+1}-x_i} (y_{i+1}-y_{i}) \\
    &=-\frac{(x-x_i)}{x_{i+1}-x_i}\frac{(x_{i+1}-x_i)^2}{2}K^{''}(\hat{\xi}_i,X_n)K^{-1}Y_n \\
    &+\frac{(x-x_i)^2}{2}K^{''}(\xi_i,X_n) K^{-1}Y_n.
\end{aligned}
\end{equation}
By Proposition \ref{lemma:K_second_derivative_K_inv}, $K^{''}(\hat{\xi}_i,X_n) K^{-1}$ is a vector with at least $n-4$ entries with absolute value smaller than $C/(n-1)$ for some constant $C$. Thus, $\|K^{''}(\xi_i,X_n) K^{-1}Y_n\|_{2}<C$ for some constant $C$ and the RHS of  \eqref{eq:higher:order}  is bounded by $ \frac{C}{(n-1)^{2}}$ for some constant $C$.
\end{proof}
After showing that $f_{\infty}^{NTK}$ can be approximated by the linear interpolation, we also need the following lemma:

\begin{lemma}[Linear Interpolation cannot Generalize Well]\label{LI_not_good}
    If $x \in [0,1]$ and $f_{\mathsf{LI}}$ is a linear interpolation estimator, then the generalization error is bounded away from zero, i.e.,
    \begin{equation}
        \int_0^1 (f_{\mathsf{LI}}(x)-f_{\star}(x))^2 dx \geq C.
  \end{equation}LI
  \end{lemma}

With Proposition \ref{LI} and Lemma \ref{thm:bad_gen}, we can prove Theorem \ref{thm:bad_gen}

\begin{proof}[Proof of Theorem \ref{thm:bad_gen}]
    \begin{equation}
        \int_0^1 (f_{\infty}^{NTK}(x)-f_{\star}(x))^2 dx \geq \int_0^1 (f_{\mathsf{LI}}(x)-f_{\star}(x))^2dx  - \int_0^1 (f_{\mathsf{LI}}(x)-f_{\infty}^{NTK}(x))^2 dx
    \end{equation}
        By Proposition \ref{LI}, $\int_0^1 ( f_{\mathsf{LI}}(x)-f_{t}^{NTK}(x))^2 dx $ is bounded by $\frac{C}{(n-1)^{4}}$. By Lemma \ref{LI}, $\int_0^1 (f_{\mathsf{LI}}(x)-f_{\star}(x))^2 dx \geq C$. To sum up, $ \int_0^1 ( f_{t}^{NTK}(x)-f_{\star}(x))^2 \geq C$.
    \end{proof}
    
    
    
%Early Stopping

==> save.11.13.NTK.tex <==


To avoid the potential confusion between positive definiteness and semi-positive definiteness, we explicitly adopt the following definition of positive definiteness of a kernel function. 
\begin{definition}
       A kernel function $K$ is strictly positive definite over domain $\mathcal{X}\subset \mathbb{R}^{d}$ if for any $n$ and any points $\bm{x}_{1},\dots,\bm{x}_{n}\in \mathcal{X}$, the smallest eigenvalue $\lambda_{\min}$ of the matrix $(K(\bm{x}_{i},\bm{x}_{j}))_{1\leq i,j\leq n}$ is strictly larger than zero.
\end{definition}

Positive definiteness of neural tangent kernel is widely assumed in literature(\cite{du2018gradient},\cite{du2019gradient},\cite{arora2019fine}). To the best of our knowledge, the positive definiteness of NTK has been only proved when it is defined on sphere $\mathbb{S}^{d}\subset \mathbb{R}^{d+1}$. The following proposition states that the NTK is strictly positive definiteness on $\mathbb{R}^{d}$. 

\begin{proposition}[Positivity of $K_{d}$]
	\label{PD}
	The neural tangent kernel $K_d(\bm{x},\bm{x}')$ is strictly positive definite on $\mathbb{R}^{d}$. Moreover, if we denote the NTK of the feedforward neural network of depth by $K_{L,d}$, we can actually show that $K_{L,d}$ is positive definite on $\mathbb{R}^{d}$ as well.
\end{proposition} 


%We have to emphasize that in order to make the neural tangent approximation hold, we need to know that $K$, the neural tangent kernel, is strictly positive definite on its domain.  This has been only proved for NTKs defined on $\mathbb{S}^{d-1}$ (\cite{jacot2018neural}). If the neural tangent kernel $K$ is strictly positive definite, then one can easily see that the gradient flow $f^{\NTK}_{t}$  in $\mathcal{F}$ will achieve the global minima. As a direct corollary, for sufficiently large $m$, the gradient flow $f_{\bm{\theta}(t)}$ in $\mathcal{F}^{m}$ will achieve the global minima with high probability.

%One of the most important observations in this study is the following: 

%\begin{remark}
%The idea of Theorem \ref{PD} is based on the fact that the inner-product kernel determined by the non-polynomial function is strictly positive definite on $\mathbb{S}^{d}_+ :=\{\bm{x}=(x_1,...,x_{d+1})\in \mathbb{S}^{d+1}\mid x_{d+1}>0\}$.
%\end{remark}

Once we know the positive definiteness of $K_{L,d}$ on $\mathbb{R}^{d}$,  we are interested in the spectral properties of $K_{L,d}$.  
In this paper, we will focus on the spectral properties of $K_{1}$ and leave the spectral properties of $K_{L,d}$ ($d>1$ and $L>1$)  to future studies. 
%want to natural to ask the spectral properties of it

%We have shown the strictly positive definiteness of NTK. The strictly positive definiteness only guarantees that $\lambda_{\min}>0$. However, the minimum eigenvalue can be related to the sample size $n$(the minimum distance), shown in Figure \ref{fig:min_eigenvalue}. For example, we can actually prove a stronger statement over data of dimension one.

%\begin{lemma}\label{min_eigenvalue} Let $X=\{x_{1},...,x_{n}\}\subset [0,\pi]$ and $d_{\min}=\min_{i\neq j}|x_{i}-x_{j}|$. The minimum eigenvalue, $\lambda_{\min}$,  of $K_1(\bm{X},\bm{X})$ satisfies that
% \begin{equation}
%  \lambda_{\min}\geq \frac{d_{\min}}{2\pi}.
%  \end{equation}
%\end{lemma}

\begin{remark}
The minimum eigenvalue of $K_1(X_{n},X_{n})$ is of particular interest in understanding the dynamics of the (very) wide neural network. Several groups of researchers studied it for high dimensional data ( e.g., \cite{ghorbani2020neural},\cite{nguyen2021tight}). Most of the works implicitly or explicitly assume that the minimum eigenvalue is a positive constant (\cite{hu2021regularization},\cite{suh2021non}). Theorem \ref{thm:spectral_properties} $i$ shows that, for the asymptotic analysis, the minimum eigenvalue depends on the sample size $n$. For example, for the equally distanced one-dimensional data, the minimum distance $d_{\min}=\frac{1}{n-1}$ and the result is shown in Figure \ref{fig:min_eigenvalue} (a). And we find that for $d>1$, the minimum eigenvalue also depends on the minimum distance, shown in Figure  \ref{fig:min_eigenvalue}.
\end{remark}


\begin{figure}[htbp]
    \begin{minipage}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\textwidth]{min_eigenvalue_d_1.png}
        \centerline{(a) $\lambda_{min}$ for the equally distanced data(d=1)}
    \end{minipage}%
    \begin{minipage}[t]{0.5\linewidth}
        \centering
        \includegraphics[width=\textwidth]{min_eigenvalue_for_diff_d.png}
        \centerline{(b) $\lambda_{min}$ for the equally distanced data(d>1)}
    \end{minipage}
    \caption{Minimum eigenvalue vs sample size(the minimum distance). (a) Let $\{x_i\}_{i=1}^n$ be the n equally-distanced one-dimensional data in [0,1], i.e., $x_i=\frac{i-1}{n-1}$ for $i\in[n]$. We calculate the minimum eigenvalue of NTK with different sample sizes $n$. (b) For $d>1$, the equally-distanced data $\{\bm{x}_i\}_{i=1}^n$ is defined as $\{(\frac{i_1-1}{n_d-1},...,\frac{i_d-1}{n_d-1})\}$, $i_1,...,i_d\in[n_d]$, where $n_d=n^{\frac{1}{d}}$. We calculate the minimum eigenvalue of NTK with different minimum distances $\frac{1}{n_d-1}$.}
    \label{fig:min_eigenvalue}
  \end{figure}

%Add 
\begin{theorem}[Spectral properties of $K_{1}$]\label{thm:spectral_properties}
The following properties hold for $K_{1}$, the neural tangent kernel defined on $[0,1]\subset \mathbb{R}$.

        $i)$ Let $X=\{x_{1},...,x_{n}\}\subset [0,\pi]$ and $d_{\min}=\min_{i\neq j}|x_{i}-x_{j}|$. The minimum eigenvalue, $\lambda_{\min}$,  of $K_1(\bm{X},\bm{X})$ satisfies that
 \begin{equation}
  \lambda_{\min}\geq \frac{d_{\min}}{2\pi}.
  \end{equation}
  
  $ii)$     Let $\{\lambda_{j}, j=0, 1,2,\cdots\}$ be the eigenvalues associated to the NTK $K_1$ defined on $[0,1]$. Then we have 
    \begin{equation}
        \frac{1}{2\pi^3} \frac{1}{j^{2}}\leq \lambda_j \leq \frac{14}{\pi^3} \frac{1}{j^{2}},~~ j=1,2,...
    \end{equation}

\end{theorem}


The decay rate of the eigenvalue can be used to analyze the reproducing kernel Hilbert space of NTK. The following lemma shows the decay rate of the eigenvalue associated with $K_1$.

%\begin{lemma}\label{lem:K_decay_rate} 
%    Let $\{\lambda_{j}, j=0, 1,2,\cdots\}$ be the eigenvalues associated to the NTK $K_1$ on $[0,1]$. Then we have 
%   \begin{equation}
%        \frac{1}{2\pi^3} \frac{1}{j^{2}}\leq \lambda_j \leq \frac{14}{\pi^3} \frac{1}{j^{2}}, j=1,2,...
%    \end{equation}
%\end{lemma}
%Add remark how to prove 
\begin{remark}
The kernel $K_1$ can be reformulated as the sum of two kernels. One is the main kernel, offering the main properties of NTK. And the proof of Theorem \ref{thm:spectral_properties} $ii$ is based on the bounds of the eigenvalues associated with the main kernel. Theorem \ref{thm:spectral_properties} $ii$ clearly shows the upper and lower bounds of the eigenvalues and indicates the size of the RKHS of NTK.  
\end{remark}

==> save.11.13.explanation.tex <==
The statement in Section \ref{sec:main_result} that neural network that overfitted neural network cannot generalize well seems to contradict the observation (S). However, we realize that it might be caused by the subtle difference between zero training label error and zero training loss. In other words, the training till zero training label error is actually stopped earlier than the time till interpolating the data. We present this subtle difference through the following illustrative example.

\begin{figure}[h]
\centering
\includegraphics[scale=0.4]{100accuracy_vs_interpolation}
\caption{Overfitting vs. 100 \% label accuracy: 4 training data points $\{(0,0),(\frac{1}{3},1),(\frac{2}{3},0), (1,1) \}$. We use gradient descent to train a one-hidden-layer neural network with large width $m=1000$. Compared with the interpolation regime, the loss in the epoch with 100 \% label accuracy is still large. The function in the epoch with 100 \% label accuracy is also far different from the function in the interpolation regime.}
\label{fig: interpolation vs acc}
\end{figure}

Although we realize the stopping time with zero training label error can be an implicit early stopping, we find that the occurrence of this implicit early stopping depends on the scale of the noise(the fraction of label corruption). In other words, the signal strength of data plays a significant role in this case.

\subsection{On the role of signal strength}

Proposition \ref{prop:early:stopping} shows that a carefully chosen early stopping time will produce a neural network  achieving the minimax rate. 
Zhang et al. \cite{zhang2016understanding} observed the implicit early stopping strategy, stopping the training process when the 100\% label accuracy is reached, can generalize well. One may speculate that the implicit early stopping time is the optimal stopping time that appeared in Proposition \ref{prop:early:stopping}. However, this sounds too good to be true. In fact, Zhang et al. \cite{zhang2016understanding} have discussed the role of some explicit early stopping strategies in training neural networks. They observed that: 1. early stopping indeed makes generalization better on ImageNet, and 2. early stopping does not help much on CIFAR10. These observations made the effects of the implicit early stopping elusive. We can not simply claim that the implicit early-stopping strategy would produce a rate-optimal neural network.

We hypothesized that signal strength plays an indispensable role in the success of implicit early-stopping strategies. More precisely, when the signal strength is strong enough, the implicit early stopping strategy will produce a stopping time near the optimal stopping time $t_{\star}$; and when the signal strength deteriorates (e.g., after performing label corruption procedure), the implicit early stopping strategy will produce a stopping time far from the optimal stopping time $t_{\star}$. 

%Talk about what is the signal strength: Smoothness and the scale of noise
%We will talk about the two reasons why the overfitted neural network can still generalize:

Experiments from \cite{belkin2018understand} show that ``early stopping provides at most a minor improvement to classifier performance'' and MNIST labels are arguably close to a deterministic function of the features, as most (but not all) digit images are easily recognizable.

\subsection{Noise of data}

%Define the scale of noise
In Section \ref{intro}, we assume the noise $\epsilon\sim N(0,\sigma)$, which is too good to be true in real cases. Nevertheless, we can still believe there is a ground-true function $f_{\star}(\bm{x})$ behind the data. Thus, we can define the gap between the label and the ground-true function as noise, i.e.,
\begin{equation}
    \epsilon = y - f_{\star}(x).
\end{equation}
In binary classification problems, the true label can be defined as
\begin{equation}
    y_{\text{true}}=\bm{1}_{f_{\star}(x)>0.5}.
\end{equation}
The labels of data $y$ are possibly different from the true labels $y_{\text{true}}$. Since the ground-true function is unknown and we actually care about the true label, we can define the small noise as followed:
\begin{definition}
    The noise of the data point $x,y$ is small if 
    \begin{equation}
        y=y_{\text{true}}
    \end{equation}
\end{definition}

For example, $f_{\star}(x_1)=0.1$ and the label $y_1=0$ and $f_{\star}(x_2)=0.6$ and the label $y_1=1$. These two data points have small noise since the gap does not affect the true labels of $f_{\star}(x_1)$ and $f_{\star}(x_2)$ even if the square losses of these two points are different. However, if the noise affects the true label, that means label corruption happens. For example, if $f_{\star}(x_3)=0.1$ but the label $y_3=1$, that means the noise affects the true label of $f_{\star}(x_3)$.

In general, the epoch with the maximum accuracy on the validation set or the long-time unchanged training loss is commonly chosen as the stopping time. In this case, early stopping is potentially used. If the neural network is trained until it reaches 100\% training accuracy, we tend to believe the network violates the conditions of early stopping and can not have a good performance on the testing set. However, even if the noise is small, 100\% training accuracy does not mean a sufficient small loss. The neural network may have a large training loss even if it reaches 100\% training accuracy, which means the training process is early stopped before the interpolation regime.

If the noise is large, the 100\%-training-accuracy neural network can not have good generalization. From Figure \ref{fig: MLP_diff_noise_mse} and \ref{fig: Alexnet_cifar10_diff_noise_ce}, we can find that as the percentage of label corruption is increasing, the training time to 100\% training accuracy is increasing. Moreover, the generalization gap between `100\% training accuracy' and `best generalization' becomes larger. In these cases, explicit early stopping(e.g. cross validation) is still significant to the generalization of the model.

In summary, we finally filled the last piece of the jigsaw in reconciling the controversial observation (S) and the bias-variance trade-off doctrine in classical statistical learning theory.



